AutoGPart: Intermediate Supervision Search for Generalizable 3D Part Segmentation

Training a generalizable 3D part segmentation network is quite challenging but of great importance in real-world applications. To tackle this problem, some works design task-specific solutions by translating human understanding of the task to machine's learning process, which faces the risk of missing the optimal strategy since machines do not necessarily understand in the exact human way. Others try to use conventional task-agnostic approaches designed for domain generalization problems with no task prior knowledge considered. To solve the above issues, we propose AutoGPart, a generic method enabling training generalizable 3D part segmentation networks with the task prior considered. AutoGPart builds a supervision space with geometric prior knowledge encoded, and lets the machine to search for the optimal supervisions from the space for a specific segmentation task automatically. Extensive experiments on three generalizable 3D part segmentation tasks are conducted to demonstrate the effectiveness and versatility of AutoGPart. We demonstrate that the performance of segmentation networks using simple backbones can be significantly improved when trained with supervisions searched by our method.

==> articles/old/exp_old.tex <==
% !TEX root = ../main.tex

\section{Experiments}

We evaluate the effectiveness of the proposed \gps to search intermediate supervisions that can be inserted in the 3D part-segmentation frameworks to improve the their domain generalization ability on three 3D part segmentation tasks: mobility-based part segmentation~\cite{yi2018deep,hu2017learning}, primitive fitting~\cite{li2019supervised,Yan_2021_ICCV,huang2021primitivenet} and semantic-based part segmentation~\cite{luo2020learning}. 
% \todo{add refs}

For each task, we demonstrate that a simple 3D point-cloud segmentation network trained by intermediate supervisions searched by \gps and segmentation task related supervisions is able to perform better than or comparable to networks trained by generic domain generalization strategies and also task-specific models proposed in previous works. 
% We demonstrate that simple 3D point-cloud segmentation networks with intermediate supervisions searched by \gps for their respective tasks could result better generalizable part segmentation networks than using generic domain generalization strategies, even outperform the delicately designed networks proposed in previous works. 
% Moreover, we try to test the effectiveness of \gps on different point-cloud processing backbones to prove its versatility. 
Moreover, we evaluate the effectiveness of \gps on two different point-cloud processing backbones (i.e. PointNet++~\cite{qi2017pointnetpp} and DGCNN~\cite{wang2019dynamic}) on mobility-based part segmentation task and primitive fitting task to demonstrate its versatility. 

% For each segmentation task, we first give it a brief overview, and then move on to the crucial details about the used datasets, compared baselines, implementation details and experimental results. 
% More details such as baseline implementation and referred code are deferred to the \textbf{supplementary material}. 
For each segmentation task, we first give it a brief overview, and then move on to datasets, compared baselines, experimental settings and analysis on experimental results. 
Some side details are deferred to the \textbf{supplemental material}.

\subsection{Mobility-based Part Segmentation}
% task; dataset; flow estimation; details;

In this section, we evaluate \gps on the mobility-based part segmentation task~\cite{yi2018deep,hu2017learning}. % e.g. deep part induction; hu et al.; and others...
Input data in this task contains two frames of an articulated object, where the shape is segmented into rigidly moving parts~\cite{yi2018deep}. 
% Points belonging to a same part have the same rigid motion pattern. 
% where points should be segmented by their respective rigid motions taken from the original shape to the transformed shape. 

% \todo{refer to previous works for the task description.}

% Next, we introduce the used datasets, compared baselines, implementation details and experimental results. 

\vpara{Datasets.}
Three datasets are used in the task: training dataset, auxiliary training dataset that is only used in the supervision search stage to help simulate domain-shift, and the out-of-domain test dataset. 
% The training dataset is created
% We give some descriptions on the used training dataset, auxiliary training dataset that is only used in the auto-search process, and the OOD-test dataset respectively in the following. 
% \vpara{Training dataset.} 

The training dataset is created from~\cite{yi2016scalable}, containing 15,776 shapes from 16 categories. 
The auxiliary dataset is created from PartNet~\cite{mo2019partnet}, containing 5,662 shapes from 4 categories  different from those used in the training dataset. 
For both of them,
we heuristically infer mobility meta-data for each shape and generate training data on-the-fly in the training process from such meta-data. 
% To generate data for training, we heuristically add some mobility as well as motion modes for each category to generate motion meta-data encoding valid motion parameters for each part. We then generate data for training on-the-fly in the training process by applying selected motions on their respective parts. 
% Note that this dataset is different from the dataset used for training in~\cite{yi2018deep}, though both of them are created from the same annotated dataset. 

% \vpara{Auxiliary training dataset.} 
% The auxiliary dataset used in the supervision searching stage is created from PartNet~\cite{mo2019partnet}, containing 5,662 shapes from 4 categories  different from those used in the training dataset. 
% Similarly, we generate motion meta-data for parts in the shape. 
% Shape pairs used in the training stage are created on-the-fly by applying selected motions on their respective parts. 
% In the training process,  based on which shapes used for training are created on-the-fly by applying selected motions on their respective parts. 
% The auxiliary dataset is only used in the auto-search process to help with domain transfer simulation. 

% \vpara{Test dataset.} 
The test dataset used is same with the one used in~\cite{yi2018deep}, which is created from~\cite{hu2017learning}, containing 875 shapes covering 175 objects from 23 categories. 
% The test dataset has only one overlapping category with the training dataset (Laptop), thus is useful for testing models' cross-domain generalization ability as stated in~\cite{yi2018deep}. 
% \todo{number of shapes; category overlap.} 


% \vpara{Baselines.} We compare out model with both task-specific baselines and task-agnostic baseline. 
% % \vpara{Task-specific methods.} 
% Task-specific baselines compared are listed as follows: 
% % We compare our model with the following baselines: 
% Deep Part Induction~\cite{yi2018deep}, JLinkage clustering (JLC)~\cite{yuan2016space} and Spectral Clustering (SC)~\cite{tzionas2016reconstructing}. 
% The performance of segmentation networks using only PointNet++ or DGCNN trained without any intermediate auxiliary supervision are also tested. 
% % network without  intermediate supervisions are also tested. 
% % Besides, we also test the performance when simply using two point cloud processing backbones without intermediate supervisions. 
% % Details about those compared baseline are deferred to the supplementary.
% % \vpara{Task-agnostic methods.} 
% Moreover, we also compare our model with two task-agnostic baselines for general domain generalization problems, namely MixStyle~\cite{zhou2021domain} and Meta-learning~\cite{li2018learning}. For both of them, we carefully implement their methods for the current task with reference to the released code. 
% % Task-agnostic baselines for general domain generalization problems 
% % We implement two task-agnostic domain generalization strategies and test their performance on this task, namely MixStyle~\cite{zhou2021domain} and Meta-learning~\cite{li2018learning}. 


% \vpara{Implementation details.}
\vpara{Experimental settings.}
We evaluate the effectiveness of \gps on two point-cloud processing backbones, namely PointNet++ and DGCNN. 
Metric used for this task is Segmentation Mean IoU (MIoU).
% Segmentation loss u
% For all three tasks, the segmentation loss used in the training stage is the negative relaxed version of the IoU score~\cite{kalogerakis20173d}. 
% To apply \gps on this task, we a
% \vpara{Flow estimation.} 
To apply \gps on this task, we add a flow estimation module ahead of the segmentation network which consumes two input point clouds to estimate deformation flow for each point in the shape. 
The estimated flow is then taken as a kind of point feature for further processing. 
% which is then taken as a kind of point feature for the following processing. 
The flow estimation module is trained following~\cite{yi2018deep}. 
We compare our method with both task-specific baselines, namely Deep Part Induction~\cite{yi2018deep}, JLinkage clustering (JLC)~\cite{yuan2016space} and Spectral Clustering (SC)~\cite{tzionas2016reconstructing}, and task-agnostic methods for domain generalization, including MixStyle~\cite{zhou2021domain} and Meta-learning~\cite{li2018learning}.

% \vpara{Auto-search stage.} 
% In the supervision searching stage, we set the batch size to 16 for both of the above mentioned backbones. 
% 100 searching epochs are performed with 4 supervisions generated from the parametric model and evaluated. 
% The parametric model is updated in each searching epoch. 

% \vpara{Evaluation stage.} 
% In the supervision evaluation stage, where the segmentation network is trained with both selected intermediate supervisions and the task related supervision, we train the model for 400 epochs. 
% % In the regular training stage, where the segmentation network is trained with both selected supervisions 
% % For \gps, we greedily choose supervisions as stated previously. We train the model for 400 epochs with the selected supervisions and the task relevant supervision. 
% MIoU values achieved on the validation set and test set at the best validation epoch are reported as in-distribution and out-distribution performance respectively. 
% % achieved on the test set at the best validation epoch is reported. 
% For learning-based baseline models, we adopt the same training and evaluation strategies with those used for our own method. 
% For others, we directly take the numbers from~\cite{yi2018deep} due to the same test set.  

% The initial learning rate is set to 0.001 for all experiments, which is dropped by 0.7 when the evaluation metric on the validation dataset has not been improved for 20 epochs. 
% We use AdaM optimization strategy for all experiments with $\beta=(0.9,0.999), eps=10^{-8}$. 
% Such setting is shared by the evaluted three tasks, and are abbreviated in the following statement. 

\vpara{Analysis on experimental results.} 
The performance of \gps and baseline models are summarized in Table~\ref{tb_res_motion_seg_eval}. 
Based on the table, we can make the following observations:
% We can observe that: 
1). \gps can outperform all task specific models by a large margin, including traditional methods (e.g. JLinkage clustering) and learning based strategies. 
2). Both \gps and task agnostic strategies for domain generalization can be combined with a point cloud processing backbone to improve its cross-domain generalization ability. 
However, as observed in Table~\ref{tb_res_motion_seg_eval}, task agnostic strategies can hardly outperform task specific strategies when using similar backbones. 
For example, PointNet++ trained using the MixStyle strategy cannot perform better than Deep Part Induction. 
A possible reason is that task prior knowledge is not properly taken into consideration in such task agnostic strategies, which may limit their expressiveness. 
In comparison, the designed parametric auxiliary supervision model takes such prior knowledge of those 3D part segmentation tasks. 
Thus, \gps is enabled to find task friendly supervisions that can help improve the generalization ability of the network better than those task agnostic strategies. 
% such task agnostic strategies do not 
% \gps can outperform all task agnostic strategies for domain generalization. 
3). 
% Adding intermediate supervisions can help improve the generalization ability of the segmentation network using a simple point cloud processing network for both DGCNN and PointNet++. 
It indicates the effectiveness of adding such intermediate supervisions on preventing the network from learning domain variant features. 
Compared with task agnostic methods which always lay much importance on gradient consistency~\cite{Mansilla_2021_ICCV}, feature alignment~\cite{zhou2021domain}, etc., we propose to add proper intermediate auxiliary supervisions to help the network learn more  generalizable and inherent features. 
Experimental results shows the effectiveness of introducing such supervisions the network's learning process. 
4). We test the effectiveness of \gps on both DGCNN and PointNet++. 
Results can show \gps is a general strategy that can be plugged in a point cloud processing network to search for its respective suitable intermediate auxiliary supervisions. 

% \subsubsection{Empirical evaluation and analysis} 


% The task should be evaluated through the performance aspect (in-distribution generalization results) and generalization aspect (out-of-distribution generalization results) w.r.t. point-cloud processing backbones' architecture and intermediate supervision. 
% To be more specific: How will different choices of backbone architectures \& intermediate supervisions influence the in-distribution and out-of-distribution generalization? 

% Results in different settings are summarized in Table~\ref{tb_res_motion_seg_eval}. 


\begin{table}[t]
    \centering
    \caption{\footnotesize Comparison of different methods on motion segmentation. 
     In-dist. and Out-of-dist. refer to In/Out-distribution generalization. 
    %  For intermediate supervision used, ``pp-conv'' denotes ``point-point contrastive loss'', ``[R, t]'' denotes ``Rigid rotation and translation prediction loss''. 
    % For convolution modules used, ``PN++'' denotes ``PointNet++ module'', ``
    } 

    \begin{tabular}{@{\;}c@{\;}|c|c@{\;}}
    \midrule
        \hline
        \specialrule{0em}{1pt}{0pt} 
        Method & In-dist. & Out-of-dist. \\ 
        \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
      
        \multirow{1}{*}{PN++} & 86.4 & 61.0
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        DGCNN~\cite{wang2019dynamic} & 88.3 & 68.1
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        MixStyle$_{\text{PN++}}$~\cite{zhou2021domain} & 86.6 & 63.4
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        MixStyle$_{\text{DGCNN}}$~\cite{zhou2021domain} & 83.1 & 69.5
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        Meta-learning$_{\text{PN++}}$~\cite{li2018learning} & 71.3 & 63.4
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        Meta-learning$_{\text{DGCNN}}$~\cite{li2018learning} & 76.5 & 69.4
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        % SeqRANSAC & N/A & 0.558
        % \\ \cline{1-3} 
        % \specialrule{0em}{1pt}{0pt}

        JLC~\cite{yuan2016space} & N/A & 67.3
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        SC~\cite{tzionas2016reconstructing} & N/A & 69.4
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        Deep Part Induction~\cite{yi2018deep} & 84.8 & 64.4
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        \gps$_{\text{PN++}}$ & \textbf{87.2} & 66.5
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        \gps$_{\text{DGCNN}}$ & 83.1 & \textbf{73.8}
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}

    \end{tabular} 
    \label{tb_res_motion_seg_eval}
\end{table} 


% \subsubsection{Automatic search results}

\eat{
\begin{table*}[t]
    \centering
    \caption{\footnotesize Auto-search results of the motion segmentation task w.r.t. point-cloud processing backbone architecture and intermediate supervision. For abbreviation used, ``Arch.'' means ``Architecture'', ``Inter. Sup.'' means ``Intermediate Supervision'', ``In-dist.'' means ``In-distribution generalization'', ``Out-of-dist.'' means ``Out-of-distribution generalization''. For intermediate supervision used, ``pp-conv'' denotes ``point-point contrastive loss'', ``[R, t]'' denotes ``Rigid rotation and translation prediction loss''. 
    } 

    \begin{tabular}{@{\;}c@{\;}|c|c|c|c@{\;}}
    \midrule
        \hline
        \specialrule{0em}{1pt}{0pt} 
        Sea. Stra. & Arch. & Inter. Sup. & In-dist. & Out-of-dist. \\ 
        \cline{1-5} 
        \specialrule{0em}{1pt}{0pt}
        
        single-branch & \multirow{2}{*}{PN++} & $2\text{mean}(\text{cross}(2N, N^2))$ & 0.856 & 0.646
        \\ \cline{1-1} \cline{3-5} 
        \specialrule{0em}{1pt}{0pt}
        
        multi-branch & ~ & $-\text{mean}(\overline{N})$ & 0.872 & 0.665
        \\ \cline{1-5} 
        \specialrule{0em}{1pt}{0pt}
      
        single-branch & \multirow{2}{*}{DGCNN} & \makecell[c]{$\overline{\text{sum}(2\cdot \text{orth}(F))}$} & 0.845 & 0.731
        \\ \cline{1-1} \cline{3-5} 
        \specialrule{0em}{1pt}{0pt}
        
        multi-branch & ~ & \makecell[c]{$(\max(-P + F^2))^2$ \\ $(\max(2\cdot F + F^2))^2$} & 0.831 & 0.738
        \\ \cline{1-5} 
        \specialrule{0em}{1pt}{0pt}
        
        % one-branch (cbd) & \makecell[c]{EC, PN++, EC} & \makecell[c]{$\overline{\max(\text{cross}(-N,-N))}$} & 0.815 & 0.681
        % \\ \cline{1-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        % two-branch & EC $\times$ 3 & \makecell[c]{$(\max(-P + F^2))^2$} & 0.830 & 0.719
        % \\ \cline{1-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        % three-branch & - & - & - & -
        % \\ \cline{1-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        % two-branch & \makecell[c]{PN++ (v2), PN++, \\ EdgeConv, PN++ (v2)} & \makecell[c]{$P^T (P - F)$, $\text{mean}(Feat)$, ${PartFeat}$} & 0.576 & 0.709
        % \\ \cline{1-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        % three-branch & \makecell[c]{PN++ (v2), EdgeConv, \\ EdgeConv, EdgeConv} & \makecell[c]{$P^T(P - F)$, $\text{mean}(Feat)$, $\text{mean}(PartFeat)$} & 0.590 & 0.733
        % \\ \cline{1-5} 
        % \specialrule{0em}{1pt}{0pt}

    \end{tabular} 
    \label{tb_res_motion_seg_search}
\end{table*} 
}

% Current results are summarized in Table~\ref{tb_res_motion_seg_search}. 

\subsection{Primitive Fitting}

In this section, we evaluate \gps on the primitive fitting task. 
Input data in this task is a single point cloud with per-point normal vector, which should be segmented based on the geometric primitives that each point belongs to. 
% \todo{task description.}

% Next, we introduce the used datasets, compared baselines, implementation details and experimental results. 

\vpara{Datasets.}
% dataset; split;
We use the same dataset with that used in~\cite{li2019supervised} in this task. To bring the task close to domain generalization setting, we split the data according to the distribution of different types of primitives in the shape. 
We use KMeans++~\cite{arthur2006k} to cluster those shapes into 7 clusters. After that, such 7 categories are then merged into 4 sets with a large distribution shift across different sets. 
Three our of four sets are taken as training dataset containing 13528 shapes in total, while the last one containing 3669 shapes is held out for OOD test. 
During the auto-search process, 3 sets in the training dataset are used for cross-validation to simulate domain shift. 
During the evaluation process, we randomly split a validation set from training dataset according to a 9:1 train-val ratio for model selection. 
More details are deferred to the supplementary material.

\vpara{Baselines.}
We compare \gps with two previous task-specific primitive fitting related works, namely SPFN~\cite{li2019supervised} and HPNet~\cite{Yan_2021_ICCV}, and three generic domain generalization methods, including Gradient Surgery (GS)~\cite{Mansilla_2021_ICCV}, MixStyle~\cite{zhou2021domain}, and Meta-learning~\cite{li2018learning}. 
More details w.r.t. the description and implementation details of such baselines are deferred to the supplementary material.


\vpara{Implementation details.}
In the automatic supervision search process,
we perform 30 epochs with 4 models generated and evaluated in each epoch. 
The parametric supervision model is optimized in each epoch. 

During the regular training stage, where the network is trained under the guidance of greedily selected supervisions from the optimized supervision model and segmentation task related supervision, we train 200 epochs for models using a classification module to propose segmentations. 
The model that achieves the highest MIoU score on the validation dataset is then taken for evaluation on the test set. 
% For models using the 
% The greedily selected supervision targets are then plugged into the segmentation framework for training and evaluation. 
% For all models using a classification module for segmentation proposal, we train the model for 200 epochs and take the model that achieves the highest MIoU score on the validation dataset for evaluation on the test set. 
For models using the Mean-Shift based clustering module to propose segmentations, we train the model for 100 epochs and take the last model for further clustering. 

\vpara{Experimental results.}
% We evaluate \gps on two point cloud processing backbones, namely PointNet++~\cite{qi2017pointnetpp} and DGCNN~\cite{wang2019dynamic}. 
The performance of \gps and other baseline models are summarized in Table~\ref{tb_prim_fit_seg_eval}. 
% The results are summarized in Table~\ref{tb_prim_fit_seg_eval}. 
We apply \gps on classification based segmentation networks, denoted by ``\gps$_{\text{PN++}}$'' and ``\gps$_{\text{DGCNN}}$'' where subscriptions indicate the used point cloud processing backbone, as well as clustering based segmentation networks used in~\cite{Yan_2021_ICCV}, denoted by ``\gps$_{\text{DGCNN}}$**''. 
When applying \gps on classification based segmentation networks, we end-to-end train the segmentation network  and use the generalization gap between valdiation dataset and trianinig dataset as the reward value. 
While when applying \gps on clustering based segmentation networks, we train the representation learning network by applying searched intermediate auxiliary supervisions along with other losses proposed in the first stage of~\cite{Yan_2021_ICCV} and use the generalization gap defined for losses as the reward value. 

We can make the following observations from Table~\ref{tb_prim_fit_seg_eval}: 
1). For classification based segmentation networks, \gps can find useful intermediate auxiliary  supervisions that can be trained together with segmentation task related loss to help significantly improve the generalization ability of the network trained using only the task related loss. 
For example, \gps can boost the performance of PointNet++ from 0.716 to 0.765 on out-of-domain test dataset.
Those results can demonstrate the effectiveness of introducing intermediate auxiliary supervisions for domain generalization improvement in one thing, and the ability of \gps to find such useful supervisions in another. 
% that can help significantly improve the generalization ability of the network
2). For classification based segmentation networks, simple networks trained under the searched intermediate supervisions and task related supervision can outperform task specific baseline models. 
For example, \gps with PointNet++ can outperform SPFN network on out-of-distribution datset. 
For clustering based segmentation networks, \gps can find useful supervisions to better regularize the representation learning process. 
3). Segmentation networks trained with auxiliary supervisions searched by \gps can outperform those trained by task-agnostic strategies such as MixStyle.

\begin{table}[t]
    \centering
    \caption{\footnotesize Evaluation of the primitive fitting task w.r.t. point-cloud processing backbone architecture. For abbreviation used, ``Arch.'' means ``Architecture'', ``Inter. Sup.'' means ``Intermediate Supervision'', ``In-dist.'' means ``In-distribution generalization'', ``Out-of-dist.'' means ``Out-of-distribution generalization''. 
    } 

    \begin{tabular}{@{\;}c@{\;}|c|c@{\;}}
    \midrule
        \hline
        \specialrule{0em}{1pt}{0pt} 
        Method & In-dist. & Out-of-dist. \\ 
        \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        ${\text{PN++}}$ & 0.815  & 0.716
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        % \rowcolor{mycyan}
        $\text{DGCNN}$ & 0.936 & 0.680
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        % $\text{SPFN}_{\text{DGCNN}}$ & 0.944 & 0.685
        % \\ \cline{1-3} 
        % \specialrule{0em}{1pt}{0pt}
        
        $\text{GS}_{\text{PN++}}$ \cite{Mansilla_2021_ICCV} & 0.907 & 0.703
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt} 
        
        $\text{GS}_{\text{DGCNN}}$ \cite{Mansilla_2021_ICCV} & 0.926 & 0.716
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt} 
        
        $\text{Meta Learning}_{\text{PN++}}$ \cite{li2018learning} & 0.650 & 0.685
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt} 

        $\text{Meta-learning}_{\text{DGCNN}}$ \cite{li2018learning} & 0.671 & 0.693
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt} 
        
        $\text{MixStyle}_{\text{PN++}}$ \cite{zhou2021domain} & 0.921 & 0.709
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt} 
        
        $\text{MixStyle}_{\text{DGCNN}}$ \cite{zhou2021domain} & 0.937 & 0.714
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt} 
        
        % $\text{Episodic Learning}_{\text{PN++}}$ \cite{li2019episodic} & 0.202 & 0.176
        % \\ \cline{1-3} 
        % \specialrule{0em}{1pt}{0pt} 
        
        % $\text{Episodic Learning}_{\text{DGCNN}}$ \cite{li2019episodic} & - & -
        % \\ \cline{1-3} 
        % \specialrule{0em}{1pt}{0pt} 
        
        $\text{SPFN}$ \cite{li2019supervised}& 0.944 & 0.723
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        HPNet* \cite{Yan_2021_ICCV} & 0.939 & 0.696
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        HPNet \cite{Yan_2021_ICCV} & N/A & 0.795
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        \gps$_{\text{PN++}}$ & 0.863 & 0.765
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        \gps$_{\text{DGCNN}}$ & 0.942 & 0.734
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        \gps$_{\text{DGCNN}}$** & N/A & 0.804
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}


    \end{tabular} 
    \label{tb_prim_fit_seg_eval}
\end{table} 

% Current results are summarized in Table~\ref{tb_prim_fit_seg_eval}.

% \subsubsection{Automatic search results}

% Primitive fitting task
\eat{
\begin{table*}[t]
    \centering
    \caption{\footnotesize Auto-search results of the primitive fitting task w.r.t. point-cloud processing backbone architecture and intermediate supervision. For abbreviation used, ``Arch.'' means ``Architecture'', ``Inter. Sup.'' means ``Intermediate Supervision'', ``In-dist.'' means ``In-distribution generalization'', ``Out-of-dist.'' means ``Out-of-distribution generalization''. For intermediate supervision used, ``pp-conv'' denotes ``point-point contrastive loss'', ``[R, t]'' denotes ``Rigid rotation and translation prediction loss''. 
    } 

    \begin{tabular}{@{\;}c@{\;}|c|c|c|c@{\;}}
    \midrule
        \hline
        \specialrule{0em}{1pt}{0pt} 
        Sear. Stra. & Arch. & Inter. Sup. & In-dist. & Out-of-dist. \\ 
        \cline{1-5} 
        \specialrule{0em}{1pt}{0pt}
      
        % one-branch & \multirow{7}{*}{PN++ $\times$ 3}  &  \makecell[c]{$\min_{\vec{c}}\Vert 2P^2\vec{c}\Vert_2$} & 0.911 & 0.691
        % \\ \cline{1-1}   \cline{3-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        % one-branch & ~ & \makecell[c]{$\min_{\vec{c}}\Vert \overline{P}\vec{c} - \text{rowsum}(\overline{P})\Vert_2$, ${P^2}^T(-N)$} & 0.910 & 0.715
        % \\ \cline{1-1}   \cline{3-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        one-branch & \multirow{3}{*}{PN++} & 
        \makecell[c]{$\overline{\text{sum}(N)}$ \\ $\overline{\text{mean}(\text{sum}(\text{cross}(-N, N^2)) + N^2)}$}
        & 0.892 & 0.742
        \\ \cline{1-1}   \cline{3-5} 
        \specialrule{0em}{1pt}{0pt}
        
        multi-branch & ~ & 
        \makecell[c]{$\overline{\text{mean}(2N - N^2)}$ \\ $\text{orth}(\text{mean}(\overline{P} \cdot \text{orth}(P)))$}
        & 0.863 & 0.765
        \\ \cline{1-1} \cline{2-2}   \cline{3-5} 
        \specialrule{0em}{1pt}{0pt}
        
        % one-branch & \multirow{7}{*}{PN++ $\times$ 3} & 
        % \makecell[c]{$\text{svd}(2P^2)$}
        % & 0.911 & 0.691
        % \\ \cline{1-1}   \cline{3-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        % one-branch & ~ & 
        % \makecell[c]{$\overline{\max(\text{orth}(N))}$ \\ $\overline{\text{sum}(P^2)}$}
        % & 0.924 & 0.724
        % \\ \cline{1-1}   \cline{3-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        % one-branch & ~ & 
        % \makecell[c]{$\text{orth}(\text{svd}(\text{cross}(N, \overline{P})))$ \\ 
        % $\overline{\max (\text{orth}(P) - \overline{N})}$
        % }
        % & 0.915 & 0.716
        % \\ \cline{1-1}   \cline{3-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        % one-branch & ~ & 
        % \makecell[c]{$(\max (P - 2N))^2$ \\ $-\text{mean}(-P\cdot (2N))$ \\ $\overline{\text{sum}(\text{cross}(-P, \text{orth}(N)))}$}
        % & 0.932 & 0.718
        % \\ \cline{1-1}   \cline{3-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        % one-branch & ~ & 
        % \makecell[c]{$-\text{svd}(\text{cross}(N,\overline{P}))$ \\ $2\cdot \max (\text{cartesian}(N^2, \overline{P}))$ \\ $-\text{svd}(-N\cdot (2P))$}
        % & 0.935 & 0.715
        % \\ \cline{1-1}   \cline{3-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        % one-branch & ~ & 
        % \makecell[c]{$\text{orth}(\text{sum}(\text{cartesian}(N^2, \overline{N})))$ \\ $\text{svd}(N^2)$ \\ $\text{sum}(\text{cartesian}(N^2, \overline{P\cdot N}))$}
        % & 0.906 & 0.731
        % \\ \cline{1-1}   \cline{3-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        % three-branch & ~ & 
        % \makecell[c]{$\overline{\text{mean}(2N)}$ \\ $(\text{sum}(P^2 - N^2))^2$ }
        % & 0.945 & 0.733
        % \\ \cline{1-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        
        % \rowcolor{mycyan} incremental search & - & - & - & - 
        % \\ \cline{1-5} 
        % \specialrule{0em}{1pt}{0pt}
        
        one-branch & \multirow{2}{*}{DGCNN}  & \makecell[c]{$(\text{mean}(\overline{N}))^2$} & 0.966 & 0.723 / (0.806)
        \\ \cline{1-1} \cline{3-5} 
        \specialrule{0em}{1pt}{0pt}
        
        multi-branch & ~ & $-\text{svd}(N)$  & 0.942 & 0.734
        \\ \cline{1-5} 
        \specialrule{0em}{1pt}{0pt}
        
        

    \end{tabular} 
    \label{tb_res_prim_fit_search}
\end{table*} 
}



% Current results are summarized in Table~\ref{tb_prim_fit_seg_eval}.


\subsection{Semantic-based Part Segmentation}
In this section, we evaluate \gps on the semantic-based part segmentation task, which is a more generic segmentation task where points are segmented into fine-grained objects' instances~\cite{mo2019partnet,luo2020learning}. 

% \todo{Task description.}

\vpara{Datasets.}
% PartNet
% most fine-grained segmentation level 
We use the same dataset provided by ~\cite{luo2020learning} as well as the train-test data splitting strategy stated in the paper. 
Specifically, 3 categories are used in the training stage, namely Chair, Lamp and Storage Furniture and the rest 21 categories are left as unseen categories for test. 
Validation dataset is further split from the training dataset via a train-val ratio 9:1. 

We adopt Mean Recall as the evaluation metric, the same one with that used in~\cite{luo2020learning}. 
Values reported in Table~\ref{tb_res_inst_seg_eval} are average Mean Recall scores over test categories. 
Detailed Mean Recall scores on each category are presented in the supplementary material to spare space. 
% Detailed values for each category are presented in the supplementary material to spare space. 


\vpara{Baselines.}
We compare \gps with four task-specific methods, including Learning to Group~\cite{luo2020learning}, SGPN~\cite{wang2018sgpn}, GSPN~\cite{yi2019gspn} and WCSeg~\cite{kaick2014shape}. 
The presented scores are taken form~\cite{luo2020learning} directly.
% Their respective values are taken from 

We also compare \gps with generic strategies for domain generalization, including MixStyle~\cite{zhou2021domain}, Meta-learning~\cite{li2018learning}. 

% \todo{gradient surgery}

\vpara{Implementation details.}
For all models, we train for 200 epochs and take the one that achieves the best performance on the validation set for further out-of-domain test. 

\vpara{Experimental results.}
The preformance of \gps and other baseline models are summarized in Table~\ref{tb_res_inst_seg_eval}. 
As shown in the table, although end-to-end learning based strategies always fail to get satisfactory results on test datasets containing shapes from unseen categories, our method can help improve their generalization ability to a level comparable to the two-stage learning based method~\cite{luo2020learning} as well as traditional segmentation methods such as WCSeg~\cite{kaick2014shape}. 
Those results demonstrate the effectiveness of the automatic supervision searching strategy in finding useful supervisions to improve learning based networks' generalization ability. 
Those results further demonstrate the effectiveness of adding intermediate auxiliary supervisions for improving the cross-domain generalization ability of learning-based segmentation networks and also the effectiveness of \gps in finding such useful supervisions. 
% targets to improve the gneerlization ability.

% \subsubsection{Empirical evaluation and analysis}

% Evaluate the in-distribution and out-distribution generalization ability when using different kinds of backbone architecture. 

% \begin{table*}[t]
%     \centering
%     \caption{\footnotesize Evaluation of the instance segmentation task w.r.t. point-cloud processing backbone architecture. For abbreviation used, ``Arch.'' means ``Architecture'', ``Inter. Sup.'' means ``Intermediate Supervision'', ``In-dist.'' means ``In-distribution generalization'', ``Out-of-dist.'' means ``Out-of-distribution generalization''. 
%     } 

%     \begin{tabular}{@{\;}c@{\;}|c|c|c|c@{\;}}
%     \midrule
%         \hline
%         \specialrule{0em}{1pt}{0pt} 
%         Arch. & \#Layers & Inter. Sup. & In-dist. & Out-of-dist. \\ 
%         \cline{1-5} 
%         \specialrule{0em}{1pt}{0pt}
%         \multirow{5}{*}{PN++} 
%         %  \rowcolor{mycyan}
%         & 3 & N/A & - & -
%         \\ \cline{2-5} 
%         \specialrule{0em}{1pt}{0pt}
        
%         % % \rowcolor{mycyan}
%         % ~ & 2 & N/A & - & -
%         % \\ \cline{2-5} 
%         % \specialrule{0em}{1pt}{0pt}
        
%         % % \rowcolor{mycyan}
%         % ~ & 1 & N/A & - & -
%         % \\ \cline{2-5} 
%         % \specialrule{0em}{1pt}{0pt}
        
%         ~ & 3 & PartNet & 0.339 & 0.267
%         \\ \cline{2-5} 
%         \specialrule{0em}{1pt}{0pt}
        
%         ~ & 1 & Learning to Group & 0.352 & 0.320
%         \\ \cline{1-5} 
%         \specialrule{0em}{1pt}{0pt}
        
%         N/A & N/A & WCSeg & 0.298 & 0.332
%         \\ \cline{1-5} 
%         \specialrule{0em}{1pt}{0pt}
        
%         % \rowcolor{mycyan}
%         % \multirow{3}{*}{EdgeConv}  & 3 & N/A & - & -
%         % \\ \cline{2-5} 
%         % \specialrule{0em}{1pt}{0pt}
        
%         % % \rowcolor{mycyan}
%         % ~ & 2 & N/A & - & -
%         % \\ \cline{2-5} 
%         % \specialrule{0em}{1pt}{0pt}
        
%         % % \rowcolor{mycyan}
%         % ~
%         % & 1 & N/A & - & -
%         % \\ \cline{1-5} 
%         % \specialrule{0em}{1pt}{0pt}

%     \end{tabular} 
%     \label{tb_res_inst_seg_eval}
% \end{table*} 

\begin{table}[t]
    \centering
    \caption{\footnotesize Evaluation of the instance segmentation task w.r.t. point-cloud processing backbone architecture. For abbreviation used, ``Arch.'' means ``Architecture'', ``Inter. Sup.'' means ``Intermediate Supervision'', ``In-dist.'' means ``In-distribution generalization'', ``Out-of-dist.'' means ``Out-of-distribution generalization''. 
    } 

    \begin{tabular}{@{\;}c@{\;}|c|c@{\;}}
    \midrule
        \hline
        \specialrule{0em}{1pt}{0pt} 
        Method & In-dist. & Out-of-dist. \\ 
        \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        % $\text{PN++}$ & - & -
        % \\ \cline{1-3} 
        % \specialrule{0em}{1pt}{0pt}
        
        PartNet-InstSeg\cite{mo2019partnet} & 0.339 & 0.267
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        MixStyle\cite{zhou2021domain} & 0.344 & 0.307
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        Meta-learning\cite{li2018learning} & 0.351 & 0.297
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        Learning to Group\cite{luo2020learning} & 0.352 & 0.320
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        SGPN\cite{wang2018sgpn} & 0.250 & 0.202
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        GSPN\cite{yi2019gspn} & 0.235 & 0.287
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        WCSeg\cite{kaick2014shape} & 0.298 & 0.332
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}
        
        \gps & 0.357 & 0.339
        \\ \cline{1-3} 
        \specialrule{0em}{1pt}{0pt}

    \end{tabular} 
    \label{tb_res_inst_seg_eval}
\end{table} 

% Current results are summarized in Table~\ref{tb_res_inst_seg_eval}.

% \subsubsection{Automatic search results}

\eat{
\begin{table*}[t]
    \centering
    \caption{\footnotesize Auto-search results of the instance segmentation task w.r.t. point-cloud processing backbone architecture and intermediate supervision. For abbreviation used, ``Arch.'' means ``Architecture'', ``Inter. Sup.'' means ``Intermediate Supervision'', ``In-dist.'' means ``In-distribution generalization'', ``Out-of-dist.'' means ``Out-of-distribution generalization''. For intermediate supervision used, ``pp-conv'' denotes ``point-point contrastive loss'', ``[R, t]'' denotes ``Rigid rotation and translation prediction loss''. 
    } 

    \begin{tabular}{@{\;}c@{\;}|c|c|c|c@{\;}}
    \midrule
        \hline
        \specialrule{0em}{1pt}{0pt} 
        Sea. Stra. & Arch. & Inter. Sup. & In-dist. & Out-of-dist. \\ 
        \cline{1-5} 
        \specialrule{0em}{1pt}{0pt}
        
        multi-branch & PN++$\times$3 & \makecell[c]{$(\text{mean}(\text{cartesian}(N, -N)))^2$ \\ $\text{sum}(\text{cartesian}(P, N^2))^2$} & 0.342 & 0.332 
        \\ \cline{1-5} 
        \specialrule{0em}{1pt}{0pt}
        
        multi-branch & PN++(v2), PN++$\times$2 & \makecell[c]{$\overline{\text{mean}(2P, (\text{mean}(-N))^2)}$ \\ $2\cdot \max(\overline{P}\cdot P^2)$} & 0.357 & 0.339
        \\ \cline{1-5} 
        \specialrule{0em}{1pt}{0pt}
        
    \end{tabular} 
    \label{tb_res_inst_seg_search}
\end{table*} 
}

% Current results are summarized in Table~\ref{tb_res_inst_seg_search}.



% \subsection{Further evaluation}
\subsection{Qualitative Evaluation}

\begin{figure*}[ht]

% insert text in the picture..
\centering
% \begin{center}
%     \footnotesize GT
% \end{center}
%     \quad 
%   \subfloat{
%     \footnotesize GT
%   }
    % \quad
    
  \subfloat{%
    \rotatebox{90}{\scriptsize{~~~~~~~~~~~~~GT}}
    \includegraphics[width=2.0cm]{./imgs/gt_7.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/gt_2.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/gt_49.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/gt_5.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/52_gt.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/gt_6.png}
    % \label{fig_prim_vis_gt_30}
    }
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/gt_38.png}
    % \label{fig_prim_vis_gt_30}
    }
    
    
% \rule[-10pt]{14.3cm}{0.05em}
\noindent\rule{\textwidth}{0.5pt}
    %\rotatebox{90}{\scriptsize{~~~~~~~~~~~~~Baseline}}
  \subfloat{%
    \rotatebox{90}{\scriptsize{~~~~~~~~~~~~~Baseline}}
    \includegraphics[width=2.0cm]{./imgs/bsl_7.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/bsl_2.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/bsl_49.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/bsl_5.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/52_bsl.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/bsl_6.png}
    % \label{fig_prim_vis_gt_30}
    }
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/bsl_38.png}
    % \label{fig_prim_vis_gt_30}
    }
    
  \subfloat{%
    \rotatebox{90}{\scriptsize{~~~~~~~~~~~~~Ours}}
    \includegraphics[width=2.0cm]{./imgs/pred_7.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/pred_2.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/pred_49.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/pred_5.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/52_pred.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/pred_6.png}
    % \label{fig_prim_vis_gt_30}
    }
  \subfloat{%
    \includegraphics[width=2.0cm]{./imgs/pred_38.png}
    % \label{fig_prim_vis_gt_30}
    }
%   \centering
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/gt_30.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/gt_12.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/gt_36_6.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/gt_32_6.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/gt_109_6.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     % \quad
% \rule[-10pt]{14.3cm}{0.05em}
    
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/bsl_30.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/bsl_12.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/bsl_36_6.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/bsl_32_6.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/bsl_109_6.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     % \quad
    
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/pred_30.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/pred_12.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/pred_36_6.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/pred_32_6.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=3cm]{./imgs/pred_109_6.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     % \quad
  
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/gt_30.png}
%     % \label{fig_prim_vis_gt_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/bsl_30.png}
%     % \label{fig_prim_vis_bsl_30}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/pred_30.png}
%     % \label{fig_prim_vis_pred_30}
%     }
    
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/gt_12.png}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/bsl_12.png}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/pred_12.png}
%     }
    
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/gt_36_6.png}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/bsl_36_6.png}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/pred_36_6.png}
%     }
    
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/gt_32_6.png}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/bsl_32_6.png}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/pred_32_6.png}
%     }
    
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/gt_109_6.png}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/bsl_109_6.png}
%     }
%     \quad
%   \subfloat{%
%     \includegraphics[width=4.5cm]{./imgs/pred_109_6.png}
%     }

  \caption{Segmentation results visualization for primitive fitting task. }
  \label{fig_exp_prim_vis}
\end{figure*}

\vpara{Segmentation visualization.}
For primitive fitting task, we compare the segmentation results achieved by applying \gps on clustering based segmentation networks (``\gps$_{\text{DGCNN}}$**'' in Table~\ref{tb_prim_fit_seg_eval}) with HPNet on shapes from test domains with a relatively large distribution shift from the training domain. 
As shown in Figure~\ref{fig_exp_prim_vis}, \gps can perform better on objects from test domains containing many planes whose primitive distributions are different from that of training domains.

\vpara{Search result visualization.}
To facilitate an intuitive understanding of the optimized parametric model, 
we draw related operator distributions of the operation tree that achieves the largest probability density value in the parametric auxiliary supervision for ``\gps$_{\text{PN++}}$'' and ``\gps$_{\text{DGCNN}}$'' on mobility-based segmentation in Figure~\ref{fig_pnpp_dgcnn_motion_space_vis}. 

% \section{Ablation Study}

% In this section, we ablate crucial components in the proposed \gps to demonstrate the effectiveness different components, including the reward function design, the expanded operants set from the input feature set, the depth of the sampling tree as well as the used unary operators and binary operators. 

% \subsection{Reward function} 
% \todo{more about generalization gap?}
% In \gps, we adopt the cross-validated average generalization gap as the reward value to estimate the effectiveness of the selected supervision target feature on improving the model's generalization ability. 
% We validate the superiority of the designed reward function by replacing it with the average metric achieved on the validation set directly and then test the performance of \gps on the motion segmentation task. 


% \todo{reward }

\begin{table}[t]
    \centering
    \caption{\footnotesize Ablation study w.r.t. the design of the parametric auxiliary parametric model the designed reward function used in the search process. 
    % For each ablations used, ``-Cross Validation'' means using a single branch train-val generalization gap as the reward value to evaluate the generalization performance of the current proposed supervision; ``-Gap'' means using only the average metric achieved on each validation set as the reward value; ``Less operatns'' denotes directly using the local part-aware geometric feature sets as input features in the parametric model without the introduced expansion to increase the diversity of the parametric model; ``Less unary operators'' means only using uanry operators from a subset of the full uanry operator set in the supervision model; ``Less binary operators'' means only using biarny operators from a subset of the full binary operator set in the supervision model; ``Less tree height'' means allowing a shallower cascaded connections between operation cells.  
    } 

    \begin{tabular}{@{\;}c@{\;}|c|c|c@{\;}}
    \midrule
        \hline
        \specialrule{0em}{1pt}{0pt} 
        Ablation & Arch. & In-dist. & Out-of-dist. \\ 
        \cline{1-4} 
        \specialrule{0em}{1pt}{0pt}
        
        / & \multirow{7}{*}{PN++} & 0.872 & 0.665
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        $-$Cross Validation & ~ & 0.856 & 0.646
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        $-$Gap & ~ & 0.906 & 0.649
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        Less operants & ~ & 0.875 & 0.631
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        Less unary operators & ~ & 0.868 & 0.641
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        Less binary operators & ~ & 0.830 & 0.651
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        Less tree height & ~ & 0.821 & 0.635
        \\ \cline{1-4} 
        \specialrule{0em}{1pt}{0pt}
        
        / & \multirow{7}{*}{DGCNN} & 0.831 & 0.738
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        $-$Cross Validation & ~ & 0.845 & 0.731
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        $-$Gap & ~ & 0.894 & 0.704
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        Less operants & ~ & 0.921 & 0.706
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        Less unary operators & ~ & 0.893 & 0.695
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        Less binary operators & ~ & 0.897 & 0.716
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        Less tree height & ~ & 0.894 & 0.718
        \\ \cline{1-4} 
        \specialrule{0em}{1pt}{0pt}
      
    \end{tabular} 
    \label{tb_res_motion_seg_search_cross_val_abl}
\end{table} 

% \begin{table*}[t]
%     \centering
%     \caption{\footnotesize Auto-search results of the motion segmentation task w.r.t. point-cloud processing backbone architecture and intermediate supervision. For abbreviation used, ``Arch.'' means ``Architecture'', ``Inter. Sup.'' means ``Intermediate Supervision'', ``In-dist.'' means ``In-distribution generalization'', ``Out-of-dist.'' means ``Out-of-distribution generalization''. For intermediate supervision used, ``pp-conv'' denotes ``point-point contrastive loss'', ``[R, t]'' denotes ``Rigid rotation and translation prediction loss''. 
%     } 

%     \begin{tabular}{@{\;}c@{\;}|c|c|c|c@{\;}}
%     \midrule
%         \hline
%         \specialrule{0em}{1pt}{0pt} 
%         Ablation & Arch. & Inter. Sup. & In-dist. & Out-of-dist. \\ 
%         \cline{1-5} 
%         \specialrule{0em}{1pt}{0pt}
        
%         / & \multirow{7}{*}{PN++} & $-\text{mean}(\overline{N})$ & 0.872 & 0.665
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         $-$Cross Validation & ~ & $2\text{mean}(\text{cross}(2N, N^2))$ & 0.856 & 0.646
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         $-$Gap & ~ & \makecell[c]{$(\text{mean}(\text{orth}(P)))^2$ \\ $(\text{mean}(N^2))^2$} & 0.906 & 0.649
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Less operants & ~ & \makecell[c]{$\overline{\max(N^2)}$ \\ $\overline{\max(2N)}$} & 0.875 & 0.631
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Less unary operators & ~ & \makecell[c]{ $(\text{mean}(\text{cartesian}(N^2, 2N)))^2$} & 0.868 & 0.641
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Less binary operators & ~ & \makecell[c]{ $-\text{mean}(\overline{N})$ \\ $\overline{\text{mean}(2\cdot N)}$} & 0.830 & 0.651
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Less tree height & ~ & \makecell[c]{$\overline{\text{sum}(-N)}$} & 0.821 & 0.635
%         \\ \cline{1-5} 
%         \specialrule{0em}{1pt}{0pt}
        
%         / & \multirow{7}{*}{DGCNN} & \makecell[c]{$(\max(-P + F^2))^2$ \\ $(\max(2\cdot F + F^2))^2$} & 0.831 & 0.738
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         $-$Cross Validation & ~ & \makecell[c]{$\overline{\text{sum}(2\cdot \text{orth}(F))}$} & 0.845 & 0.731
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         $-$Gap & ~ & \makecell[c]{$\overline{\max((2\cdot N) \cdot N )}$} & 0.894 & 0.704
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Less operants & ~ & \makecell[c]{$\overline{\text{mean}(\text{cartesian}(2\cdot N, 2\cdot P))}$ \\ $\text{mean}(2\cdot N - P)$ \\ $\overline{\text{mean}(\text{cartesian}(-N, \text{orth}(N)))}$} & 0.921 & 0.706
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Less unary operators & ~ & \makecell[c]{$(\text{mean}(2\cdot N))^2$ \\ $(\text{mean}(N))^2$} & 0.893 & 0.695
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Less binary operators & ~ & \makecell[c]{$\overline{\max(-N)}$ \\ $\overline{\max(-P)}$ \\ $\overline{\max(-(P-N))}$} & 0.897 & 0.716
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Less tree height & ~ & \makecell[c]{$\overline{\max(N-P)}$ \\ $(\text{mean}(\overline{N}))^2$ \\ $(\text{mean}(2\cdot(P\cdot N)))^2$} & 0.894 & 0.718
%         \\ \cline{1-5} 
%         \specialrule{0em}{1pt}{0pt}
      
%         % / & \multirow{2}{*}{DGCNN} & \makecell[c]{$(\max(-P + F^2))^2$ \\ $(\max(2\cdot F + F^2))^2$} & 0.831 & 0.738
%         % \\ \cline{1-1} \cline{3-5} 
%         % \specialrule{0em}{1pt}{0pt}
        
%         % $-$Cross Validation & ~ & \makecell[c]{$\overline{\text{sum}(2\cdot \text{orth}(F))}$} & 0.845 & 0.731
%         % \\ \cline{1-5} 
%         % \specialrule{0em}{1pt}{0pt}

%     \end{tabular} 
%     \label{tb_res_motion_seg_search_cross_val_abl}
% \end{table*} 


\begin{figure*}[ht]
  \centering
  \subfloat{%
    \includegraphics[width=4.5cm]{./imgs/prim_dgcnn_cluster_1.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=4.5cm]{./imgs/prim_dgcnn_cluster_2.png}
    % \label{fig_prim_vis_bsl_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=4.5cm]{./imgs/prim_dgcnn_cluster_3.png}
    % \label{fig_prim_vis_pred_30}
    }
%     \quad
%   \subfloat{%
%     \includegraphics[width=4cm]{./imgs/dgcnn-prim-cluster-4.png}
%     % \label{fig_prim_vis_pred_30}
%     }
  
  \caption{Segmentation results visualization for primitive fitting task for \gps using DGCNN as the backbone. }
  \label{fig_exp_prim_dgcnn_part_cluster_vis}
\end{figure*}

\begin{figure*}[ht]
  \centering
  \subfloat{%
    \includegraphics[width=4.5cm]{./imgs/prim_pnpp_cluster_1.png}
    % \label{fig_prim_vis_gt_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=4.5cm]{./imgs/prim_pnpp_cluster_2.png}
    % \label{fig_prim_vis_bsl_30}
    }
    \quad
  \subfloat{%
    \includegraphics[width=4.5cm]{./imgs/prim_pnpp_cluster_3.png}
    % \label{fig_prim_vis_pred_30}
    }
%     \quad
%   \subfloat{%
%     \includegraphics[width=4cm]{./imgs/dgcnn-prim-cluster-4.png}
%     % \label{fig_prim_vis_pred_30}
%     }
  
  \caption{Segmentation results visualization for primitive fitting task for \gps using PointNet++ as the backbone. }
  \label{fig_exp_prim_pnpp_part_cluster_vis}
\end{figure*}


\begin{figure}[ht]
  \centering
  \subfloat[PointNet++ with \gps]{%
    \includegraphics[width=3.8cm]{./imgs/pnpp_motion_res_dist.pdf}
    }
    \quad
  \subfloat[DGCNN with \gps]{%
    \includegraphics[width=3.8cm]{./imgs/dgcnn_motion_res_dist.pdf}
    }
  \caption{Vis. of optimized distributions.}
  \label{fig_pnpp_dgcnn_motion_space_vis}
\end{figure}

% \subsubsection{Segmentation visualization}
% \todo{Comparison}

% \subsubsection{Search result visualization }

% \todo{segmentation results visualization?}


\section{Ablation Study}

In this section, we ablate crucial components in the proposed \gps to demonstrate the effectiveness of such components, including the reward function design, the parametric model design, and the supervision combination selection strategy. 
% the expanded operants set from the input feature set, the depth of the sampling tree as well as the used unary operators and binary operators. 

Experimental results w.r.t. reward function design and the parametric model design are summarized in Table~\ref{tb_res_motion_seg_search_cross_val_abl}. 
Those regarding to the supervision combination selection strategy are summarized in Table~\ref{tb_res_motion_seg_search_sup_sel_stra}. 

\subsection{Reward Function Design} 
\todo{more about generalization gap?}
In \gps, we adopt the cross-validated average generalization gap as the reward value to estimate the effectiveness of the selected supervision on improving the model's generalization ability. 
We validate the superiority of the designed reward function by replacing it with the average metric achieved on the validation set directly and then test the performance of \gps on the motion segmentation task. 
We validate the superiority of the designed reward function by replacing it with 1). single branch generalization gap (denoted as ``-Cross validation'' in Table~\ref{tb_res_motion_seg_search_cross_val_abl}), and 2). average performance on the validation set over all splits (denoted as ``-Gap'' in Table~\ref{tb_res_motion_seg_search_cross_val_abl}). 
% \todo{reward }

\subsection{Supervision target space design}

To demonstrate the necessity of enough diversity of the designed supervision space, 
To demonstrate the superiority of a diverse supervision space, we downsize the supervision space by downsizing the input local part-aware geometric feature set, the uanry operator set and the binary operator set respectively and then evaluating the effectiveness of the searched supervision combinations. 

% To demonstrate the necessity of a large feature generation space, we ablate its components by using  subsets of their corresponding original sets and test the performance of \gps when using such smaller feature spaces. 

We ablate the diversity of the parametric model from the following three aspects: 
\begin{itemize}
    % \item Replace the operant set from the original one expanded from the input feature set with the input feature set directly; 
    \item Replace the input local part-aware geometric set expanded from the input feature set with a feature set containing only input geometric features, denoted as ``Less operants'' in Table~\ref{tb_res_motion_seg_search_cross_val_abl};
    \item Replace the uanry operator set with its subset, denoted as ``Less unary operators'' in Table~\ref{tb_res_motion_seg_search_cross_val_abl};
    \item Replace the binary operator set with its subset, dentoed as ``Less bianry operators'' in Table~\ref{tb_res_motion_seg_search_cross_val_abl};  
    \item Set the maximum connection number between operation cells from 3 to 2, denoted as ``Less tree height'' in Table~\ref{tb_res_motion_seg_search_cross_val_abl}. 
    % \item Set the maximum height of the feature generation tree from 3 to 2, thus the feature generated from the operation space may be less complex than those generated from the original space. 
\end{itemize} 
Details w.r.t. ablated version of each component are deferred to the supplementary material. 

% Specifically, the small unary operator set used is \{Identity, Square, Double, Negative\}; the small binary operator set used is \{Add, Minus, Multiply\}; the small operant set  used is the input feature set of size 2. 
% \todo{input feature set for each task --- talk about estimated normal vector used in instance segmentation task. }

% Followings are candidates to ablate: 
% \begin{itemize}
%     \item Whether expand the input feature set; 
%     \item Maximum height of the target tree;
%     \item Unary operator \& binary operator set. 
% \end{itemize}

\subsection{Supervision target combination selection strategy}

After the parametric auxiliary supervision model has been optimized, we adopt a greedy selection strategy to select supervision combinations that achieve the best cross-validation performance from the optimized space. 
To demonstrate the effectiveness of the greedy selection strategy, we try ablate it and adopt the following two selection strategies: 1). Directly choose top $K (1\le K \le 3)$ features from the ordered feature set ranked by the probability density value and then add intermediate supervisions based on such features. Results of the above mentioned ablated versions are summarized in Table~\ref{tb_res_motion_seg_search_sup_sel_stra}. 
2). Randomly choose features from the optimized parametric model. 
We randomly select ten supervisions from the parametric model for both PointNet++ and DGCNN and then evaluate their cross-dmain generalization performacne. 
Results are plot in Figure~\ref{fig_abl_random_pnpp_dgcnn}.
% To demonstrate the effectiveness of the greedy selection strategy, we replace it by directly selecting top K ($K\in \{1,2,3\}$) features that achieve largest possibility density value from the optimized distributions and test their performance. 
% The results are summarized in Table~\ref{tb_res_motion_seg_search_sup_sel_stra}


% \todo{a graph for random selection...}


% \begin{table*}[t]
%     \centering
%     \caption{\footnotesize Auto-search results of the motion segmentation task w.r.t. point-cloud processing backbone architecture and intermediate supervision. For abbreviation used, ``Arch.'' means ``Architecture'', ``Inter. Sup.'' means ``Intermediate Supervision'', ``In-dist.'' means ``In-distribution generalization'', ``Out-of-dist.'' means ``Out-of-distribution generalization''. For intermediate supervision used, ``pp-conv'' denotes ``point-point contrastive loss'', ``[R, t]'' denotes ``Rigid rotation and translation prediction loss''. 
%     } 

%     \begin{tabular}{@{\;}c@{\;}|c|c|c|c@{\;}}
%     \midrule
%         \hline
%         \specialrule{0em}{1pt}{0pt} 
%         Ablation & Arch. & Inter. Sup. & In-dist. & Out-of-dist. \\ 
%         \cline{1-5} 
%         \specialrule{0em}{1pt}{0pt}
        
%         Beam Search & \multirow{4}{*}{PN++} & \makecell[c]{$-\text{mean}(\overline{N})$}  & 0.872 & 0.665
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Top1 & ~ & $\overline{\max(N\cdot \overline{N})}$  & 0.871 & 0.656
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
      
%         Top2 & ~  & \makecell[c]{$\overline{\max(N\cdot \overline{N})}$ \\ $-\text{mean}(\overline{N})$}  & 0.815 & 0.645
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Top3 & ~ & \makecell[c]{$\overline{\max(N\cdot \overline{N})}$ \\ $-\text{mean}(\overline{N})$ \\ $\overline{\max(\overline{P}\cdot(-P))}$} &  0.858 & 0.628
%         \\ \cline{1-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Random1 & \multirow{3}{*}{PN++} & -  & - & -
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
      
%         Random2 & ~  & -  & - & -
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Random3 & ~ & - & - & - 
%         \\ \cline{1-5}
%         \specialrule{0em}{1pt}{0pt}

%     \end{tabular} 
%     \label{tb_res_motion_seg_search_sup_sel_stra}
% \end{table*}

\begin{table}[t]
    \centering
    \caption{\footnotesize
    Ablation study w.r.t. the supervision combination selection strategy. 
    } 

    \begin{tabular}{@{\;}c@{\;}|c|c|c@{\;}}
    \midrule
        \hline
        \specialrule{0em}{1pt}{0pt} 
        Ablation & Arch. & In-dist. & Out-of-dist. \\ 
        \cline{1-4} 
        \specialrule{0em}{1pt}{0pt}
        
        Beam Search & \multirow{4}{*}{DGCNN}  & 0.831 & 0.738
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        Top1 & ~ & 0.921 & 0.701
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
      
        Top2 & ~  & 0.898 & 0.678
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        Top3 & ~ &  0.907 & 0.716
        \\ \cline{1-4}
        \specialrule{0em}{1pt}{0pt}
        
        Beam Search & \multirow{4}{*}{PN++} & 0.872 & 0.665
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        Top1 & ~  & 0.871 & 0.656
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
      
        Top2 & ~  & 0.815 & 0.645
        \\ \cline{1-1} \cline{3-4}
        \specialrule{0em}{1pt}{0pt}
        
        Top3 & ~ &  0.858 & 0.628
        \\ \cline{1-4}
        \specialrule{0em}{1pt}{0pt}

    \end{tabular} 
    \label{tb_res_motion_seg_search_sup_sel_stra}
\end{table}

% \begin{table*}[t]
%     \centering
%     \caption{\footnotesize Auto-search results of the motion segmentation task w.r.t. point-cloud processing backbone architecture and intermediate supervision. For abbreviation used, ``Arch.'' means ``Architecture'', ``Inter. Sup.'' means ``Intermediate Supervision'', ``In-dist.'' means ``In-distribution generalization'', ``Out-of-dist.'' means ``Out-of-distribution generalization''. For intermediate supervision used, ``pp-conv'' denotes ``point-point contrastive loss'', ``[R, t]'' denotes ``Rigid rotation and translation prediction loss''. 
%     } 

%     \begin{tabular}{@{\;}c@{\;}|c|c|c|c@{\;}}
%     \midrule
%         \hline
%         \specialrule{0em}{1pt}{0pt} 
%         Ablation & Arch. & Inter. Sup. & In-dist. & Out-of-dist. \\ 
%         \cline{1-5} 
%         \specialrule{0em}{1pt}{0pt}
        
%         % Beam Search & \multirow{4}{*}{PN++} & $-\text{mean}(\overline{N})$ & 0.872 & 0.665
%         % \\ \cline{1-1} \cline{3-5}
        
%         % Top1 & ~ & -  & - & -
%         % \\ \cline{1-1} \cline{3-5}
%         % \specialrule{0em}{1pt}{0pt}
      
%         % Top2 & ~  & -  & - & -
%         % \\ \cline{1-1} \cline{3-5}
%         % \specialrule{0em}{1pt}{0pt}
        
%         % Top3 & ~ & - & - & - 
%         % \\ \cline{1-5}
%         % \specialrule{0em}{1pt}{0pt}
        
%         Beam Search & \multirow{4}{*}{DGCNN} & \makecell[c]{$(\max(-P + F^2))^2$ \\ $(\max(2\cdot F + F^2))^2$}  & 0.831 & 0.738
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Top1 & ~ & $-\text{sum}(\overline{N}\cdot \overline{N})$  & 0.921 & 0.701
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
      
%         Top2 & ~  & \makecell[c]{$-\text{sum}(\overline{N}\cdot \overline{N})$ \\ $(\max(2N + N^2))^2$ }  & 0.898 & 0.678
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Top3 & ~ & \makecell[c]{$-\text{sum}(\overline{N}\cdot \overline{N})$ \\ $(\max(2N + N^2))^2$ \\ $(\max(-P + N^2))^2$} &  0.907 & 0.716
%         \\ \cline{1-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Beam Search & \multirow{4}{*}{PN++} & \makecell[c]{$-\text{mean}(\overline{N})$}  & 0.872 & 0.665
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Top1 & ~ & $\overline{\max(N\cdot \overline{N})}$  & 0.871 & 0.656
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
      
%         Top2 & ~  & \makecell[c]{$\overline{\max(N\cdot \overline{N})}$ \\ $-\text{mean}(\overline{N})$}  & 0.815 & 0.645
%         \\ \cline{1-1} \cline{3-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         Top3 & ~ & \makecell[c]{$\overline{\max(N\cdot \overline{N})}$ \\ $-\text{mean}(\overline{N})$ \\ $\overline{\max(\overline{P}\cdot(-P))}$} &  0.858 & 0.628
%         \\ \cline{1-5}
%         \specialrule{0em}{1pt}{0pt}
        
%         % Random1 & \multirow{3}{*}{DGCNN} & -  & - & -
%         % \\ \cline{1-1} \cline{3-5}
%         % \specialrule{0em}{1pt}{0pt}
      
%         % Random2 & ~  & -  & - & -
%         % \\ \cline{1-1} \cline{3-5}
%         % \specialrule{0em}{1pt}{0pt}
        
%         % Random3 & ~ & - & - & - 
%         % \\ \cline{1-5}
%         % \specialrule{0em}{1pt}{0pt}

%     \end{tabular} 
%     \label{tb_res_motion_seg_search_sup_sel_stra}
% \end{table*}

% \begin{figure}[ht]
%   \centering
%     \includegraphics[width=0.9\linewidth]{./imgs/random_edgeconv.pdf}

%   \caption{Comparison between the performance achieved by supervision targets combination selected by our strategy and randomly selected targets from the optimized supervision distribution space.}
%   \label{fig_abl_random_ec}
% \end{figure}

% \begin{figure}[ht]
%   \centering
%     \includegraphics[width=0.9\linewidth]{./imgs/random_pnpp.pdf}

%   \caption{Comparison between the performance achieved by supervision targets combination selected by our strategy and randomly selected targets from the optimized supervision distribution space.}
%   \label{fig_abl_random_pnpp}
% \end{figure}



% \todo{Random model ---- sample k models and draw an img}

\begin{figure}[ht]
  \centering
  \subfloat[PointNet++]{%
    \includegraphics[width=0.46\linewidth]{./imgs/random_pnpp-2.pdf}
    }
    \quad
  \subfloat[DGCNN]{%
    \includegraphics[width=0.46\linewidth]{./imgs/random_dgcnn-2.pdf}
    }
  \caption{Comparison between the performance achieved by the supervision  combination selected by our strategy and randomly selected supervision from the optimized parametric model.}
  \label{fig_abl_random_pnpp_dgcnn}
\end{figure}


==> articles/old/intro_old.tex <==
% !TEX root = ../main.tex

\section{Introduction}
\label{sec:intro}

\begin{figure}[ht]
  \centering
    \includegraphics[width=0.5\textwidth]{./imgs/overview.pdf}
  \caption{Overview of \gps.}
  \label{fig_task_overview}
\end{figure}

3D part segmentation tasks have gain wide attention and interest over the past several years for their wide applications~\cite{Yan_2021_ICCV,li2019supervised,luo2020learning,yi2018deep,mo2019partnet,huang2021primitivenet,le2021cpfn,hu2012co,hu2017learning,liu2017sgn}.
There are a number of ways to define parts which may vary under different applications, like geometric primitives~\cite{Yan_2021_ICCV,li2019supervised,huang2021primitivenet}, rigid motions take  from the original shape to the transformed shape~\cite{yi2018deep,hu2012co,hu2017learning}, or via semantic information and space distance~\cite{luo2020learning,mo2019partnet,liu2017sgn}.
Previous works have devote heavy efforts on high performance 3D part-segmentation neural networks~\cite{huang2021primitivenet,Yan_2021_ICCV,li2019supervised,yi2018deep}.
Furthermore, there is also a pile of works trying to solve such problems under the domain generalization/zero-shot scenarios, where the segmentation network is trained on one or several domains while being expected to generalize to out-of-domain objects, such as generalizing to unseen object categories~\cite{yi2018deep,luo2020learning}.
Designing generalizable part segmentation networks is not an easy thing, especially when domain specific information could provide spurious cues, but easy for the network to be aware of, for segmentation results. 
Specifically, shape related information that would disappear in out-of-domain (OOD) test datasets is a good example for such spurious cues. 
As observed in~\cite{luo2020learning}, the trained 3D part segmentation network always tend to get unsatisfactory performance on shapes from unseen categories, while it can output good segmentation results on shapes from seen categories. 
\todo{the importance of training generalizable part-segmentation networks?}
% As observed in previous works, ...\todo{add examples in previous works}
\todo{DG literatures?}


Designing generalizable part-segmentation networks always requires domain knowledge of that specific segmentation task, which is further used by researchers to add more inductive bias to the design of the network. % to guide  the learning process of the segmentation network such that the network can learn how to segment parts more ``correctly''. 
% For example... \todo{previous trails and designs}
Take HPNet~\cite{Yan_2021_ICCV} as an example, where the network is designed to ... \todo{briefly summarize the design of HPNet.}
Approaches of another stream are those generic domain generalization strategies that can be plugged in the network for each segmentation task~\cite{li2018learning,li2019episodic,Mansilla_2021_ICCV,zhou2021domain,wang2021generalizing,rosenfeld2020risks,blanchard2017domain}. 
% can be seen as generic domain generalization strategies, which are task-agnostic and can be plugged in the network for each segmentation task. 


However, there are potential drawbacks of both the above mentioned strategies. 
On the first hand, task specific strategies always require researchers to have a deep understanding of the current task, which should be further translated to guide the learning process of the network, including the framework structure and how to supervise, into the network design. 
Such a process often means heavy human interference as well as a huge mount of trail-and-errors to find optimal solutions. 
Moreover, sometimes the understanding from human w.r.t. the correct way by which the network should learn to solve the task inherently cannot align well with the comfortable ways that machines usually prefer to. 
% Take the rotation prediction as an example, 
% \todo{add example, perhaps rotation prediction?}
Therefore, such approaches are neither human-time efficient, nor well guaranteed to find an optimal solution due to the limited human knowledge space. 

On the other hand, as for those model-agnostic strategies which are supposed to consistently contribute to the generalization ability of segmentation networks, they neglect prior task related knowledge that can help improve the performance of the network, if being used properly, since their general to different kinds of tasks limit the design space that can be modified of the network. 
Such limitation may restrict the capability of the resulting network, thus perhaps indicating their hard to reach a comparable level as task-specific methods. 
% indicates the restricted ability of the network. 
% prior knowledge about the task is hard  task knowledge cannot be used properly in such strategies  the generalization performance of segmentation networks for all those tasks, their approaches always focus on common part of the network such as modifying gradients. 
% Such limitation indicates the restricted ability not enough to solve the problem to a comparable level as with task-specific methods. 

Therefore, in this work, we propose a task-category level auto-learning solution, which is composed of a fixed segmentation framework with a flexible parts from which auxiliary supervisions generated to better guide and regularize the learning of the network. 
Specifically, we fix the form of adding auxiliary supervisions to minimizing the L2-distance between the projected per-point representations and features selected from a feature generation space designed particularly for 3D part segmentation tasks. 
% 
We adopt a reinforcement learning based approach to optimize the supervision target features space for each segmentation task. 
After the optimization, we greedily select features from the space based on the generalization performance estimated by the cross validation to simulate the out-of-domain transfer. 
% a fixed segmentation  and a flexible part which chooses what features to learn, and thus what supervisions to use to guide the learning process of the network particularly for the task. 
Such a design enables us to keep strengths of the above mentioned two previous solutions, while avoiding their potential drawbacks at the same time. 
Firstly, the task category level prior knowledge is added to the design of the supervision target feature space, which restrict the feature space to be task-meaningful. 
% Firstly, the supervision search space is designed particularly for 3D part-segmentation tasks which is aware of and thus at the same time contains many geometric features, with the knowledge that local geometric features are domain-invariant and are useful for segmentation tasks. 
% dynamically for the task.  that is universal for 3D part-segmentation tasks which automatically finds what features to learn for generalizable segmentation networks. 
% Such task-category solution can have both the advantages of the above mentioned two strategies. 
% Firstly, with a design space, the designed space permit a bit of flexibility that enables us to find optimal networks for each task. 
Secondly, both the limitation and human time consuming features of hand-designed framework can be alleviated when equipped with the automatic supervision search strategy to find useful auxiliary supervisions automatically for its convenience and the enlarged feature space broader than the hand-crafted one. 
% Secondly, human efforts needed in the network design process can be alleviated to some extend when equipped with the automatic supervision search strategy. 
% Moreover, it is possible that such strategy can help us get better supervisions than hand designed ones due to the enlarged search space which may contain more and also better supervisions. 
We demonstrate that, using simple segmentation networks with the auxiliary supervisions added based on the searched supervision target features, we can get better or comparable performance compared with previous delicately designed task-specific approaches as well as when using generic domain generalization strategies. 
% networks with same point-cloud processing backbone using generic methods to enhance domain generlization ability. 
% Moreover, the design space is designed to be aware of geometric features, which are domain-agnostic information and are useful for 3D part segmentation tasks.

To summarize, our contributions lie in the following aspects: 
1). A geometry aware supervision target space for supervision search. 
2). A 3D part segmentation framework which can automatically find which what intermediate supervisions to add in the training process that is universally effective for the evaluated three segmentation tasks. 
Moreover, it is a promising direction to include more parts of the network design process in the automatic search space, such as the network topology, moving the AutoML community to a new direction not limited to the current explored space, like NAS, auto-loss function, auto-augmentation. 




==> articles/old/method_old.tex <==
% !TEX root = ../main.tex

\section{Method}

\subsection{Pipeline overview}

\begin{figure*}[ht]
  \centering
    \includegraphics[width=0.9\textwidth]{./imgs/overall-pipeline-5.pdf}
  \caption{Overall pipeline of \gps.}
  \label{fig_overall_pipeline}
\end{figure*}



Aiming to develop a general framework to solve 3D part segmentation problems effectively under the domain generalization setting, we design our model into a lightweight point-cloud segmentation network plus the flexible intermediate supervisions added on each node's intermediate representations.
The overall pipeline is shown in Fig~\ref{fig_overall_pipeline}.

The point-cloud segmentation network is fixed for all kinds of segmentation tasks, while what intermediate supervisions to add is a flexible part that many be different for each task. 

In order to find such intermediate supervisions for each segmentation task that can help with improving the generalization ability of the segmentation network, we propose a supervision target space which is the optimized to fit each task. 
After the space is optimized, we adopt a certain strategy to select what kinds of supervision targets to use for the current segmentation task.

Next, we will introduce the design details of the supervision target design, how the space is optimized, how we choose what supervision to use from the optimized space as well as some qualitative evaluations of features contained in the space. 

\subsection{Supervision target space}

% \todo{The relationship between the designed space and point cloud geometry}

% hwo the tree is constructed? 
% tree nodes ---- node space
% how nodes are connected? --- node connection space --- the operation flow

Based on the observation that such intermediate supervision targets' formula can be decomposed to a sequence of simple operators applied on geometry features gradually, we model a formula as an operation tree. 
Then the target space contains a sequential conditional operator distributions, from which we can sample a sequence of operators that are further used to define an operator tree to generate the supervision target to train the model. 

Moreover, the maximum height of the operation tree is limited to restrict the complexity of the generated supervision target to a reasonable range.

Next we will introduce the structure of the operation tree by introducing each kind of operation cell structure (node structure) and operation flow structure (how nodes are connected in the tree). 

\subsubsection{Operation cell space}

\begin{table*}[t]
    \centering
    \caption{\footnotesize Valid choices of different kinds of operators used in the construction of our supervision target space, where grouping operators operate on a set of point features, binary and unary operators operate on features from a single point. 
    For grouping operators, ``SVD'' means ``Singular Value Decomposition'', where a matrix formed by features from a set of points is decomposed, whose right singular matrix is taken as the grouped feature matrix. 
    } 

    \begin{tabular}{@{\;}c@{\;}|c@{\;}}
    \midrule
        % \toprule
        \hline
        \specialrule{0em}{1pt}{0pt} 
        Operators & Choices \\ 
        \cline{1-2} 
        \specialrule{0em}{1pt}{0pt}
        Grouping operators & Sum, Average, Maximum, SVD
        \\ \cline{1-2} 
        \specialrule{0em}{1pt}{0pt}
        
        Binary operators & \makecell[c]{Add, Minus, Multiply, Cross Product, \\ Cartesian Product, Matrix-vector Product} 
        \\ \cline{1-2} 
        \specialrule{0em}{1pt}{0pt}
        
        Unary operators &  Identity, Square, Double, Negative, Orthogonalize, Inverse
        \\ \cline{1-2} 
        \specialrule{0em}{1pt}{0pt}

    \end{tabular} 
    \label{tb_method_tree_gen_ops}
\end{table*} 

\begin{figure}[ht]
  \centering
    \includegraphics[width=\linewidth]{./imgs/cell-tree-structure-and-sampling-4.pdf}

  \caption{Illustration of the cell structure, the top-down sampling process, the calculate }
  \label{fig_overall_cell_structure_and_sampling}
\end{figure}

% \todo{Geometry meanings by some examples w.r.t. what can be calculated our from such space? }

Before we introduce the operation cell structure, we first give some illustrations w.r.t. basic components of tree nodes -- operator nodes and operant nodes. 
Three kinds of operator nodes are defined in our space, namely grouping operator nodes (i.e., $g\in \mathcal{G}$), unary operator nodes (i.e., $u\in \mathcal{U}$) and bianry opeartor nodes (i.e., $b\in \mathcal{B}$) as shown in Table~\ref{tb_method_tree_gen_ops}, which are relatively basic ones operating on a set of point features or features of a single point.
Each operator node contains a set of possible operators and multinominal distribution describing the preference to such operators. 
Operant nodes contains a set of point-level features expanded from the input feature set by adding some point-level features calculated based on input features as well as a multinomial distribution indicating the preference of this node to those different operants. 
% are chosen from a feature set which is expanded from the input feature by adding some point-level features calculated based on input features. 

Then, operation cells are formed by piling up such operator nodes and operant nodes for operation sequences. 
Cells can be divided into two kinds, mid-level cells and leaf cells.
Each mid-level cell is composed of a unary operator node and $\vert \mathcal{U} \vert$ grouping operator nodes. 
Each leaf cell is composed of a uanry operator node and $\vert \mathcal{U} \vert$ operant nodes. 

% \todo{add two figures, the first one should draw the cell structure, the second one depicts how they are connected together.}



\subsubsection{Operation flow space}

Based on the above defined cell structures, the operation sampling is the constructed by connecting cells of different kinds together with distributions controlling which connection to use in the operation tree sampling process. 
The operation flow space is formed by such distributions. 

Specifically, for each mid-level operation cell, we add a children selection distribution for each of its $(u, g)$ combination. 
This distribution determines which kinds of children cells to add for this cell. 
We add a restriction that there must be at least one leaf cell child to guarantee at least one input to the mid-level operation cell a point-level feature. 
Take an mid-level cell with height $h$ as an example, its children can be chosen from \{[a leaf cell], [a leaf cell, a mid-level cell with height $h-1$], [a mid-level cell with height $h-1$, a leaf cell], [a leaf cell, a leaf cell]\}. 

% In order to automatically choose what supervisions to use in the learning process, we need to design a learnable supervision generation space and generate such features from it. Next we will introduce how we design our supervision space and how we sample from it. 

% \subsubsection{Space design}

% To make the supervision learnable, we model the supervision target feature generation process as a multi-step operators and operants selection process. We sample a sequence of operators from the constructed space and use them to generate the supervision target feature by applying them on the selected input operants step by step. 

% Three kinds of operators are included in the space, which are grouping operators, binary operators and unary operators. Grouping operators operate on a set of point features, aiming at summarizing them into a single feature. The remaining operators operate on features from a single point by transforming them to a new feature vector. Choices of such such three operators designed in our space are summarized in Table~\ref{tb_method_tree_gen_ops}. 

% Based on the definition of operators and operants, the supervision space can be spanned into an operation tree, where we first define tree nodes from different levels by fixing certain operation combinations in them which are further organized into a supervision target formula generation tree. 

% Due the construction time which may be shored up when the maximum height of the operation tree increases as well as for the purpose to limit the supervision target space, and further the optimization difficulty, we set a maximum height of the supervision target generation tree to 3. 
% Therefore, nodes of three different levels are defined in the following: 
% \begin{itemize}
%     \item Level 1 node (the highest node which is nearest to the output): It is composed of a unary operator distribution and a grouping operator distribution. Children of such nodes are chosen from \{[a level-3 node], [a level-2 node, a level-2 node], [a level-2 node, a level-3 node], [a level-3 node, a level-2 node]\}. 
%     \item Level 2 node: It is composed of a unary operator distribution and a grouping operator distribution. Children of such nodes are chosen from \{[a level-3 node], [a level-3 node, a level-3 node]\}. 
%     \item Level 3 node: It is composed of a unary operator distribution and an input feature operant distribution. 
%     % \item Input feature operant node: Operant is sampled from the expand input feature set. 
% \end{itemize}

% Then, the sampling tree is constructed gradually by adding deeper level nodes on shallower nodes for each possible shallower operation combination. 





% To be more specific, we first sample components of the highest node, including its grouping operator and the unary operator from their respective multinomial distribution. 
% After that, we sample its children from its corresponding distribution. 
% Then, we gradually nodes in lower levels by sampling their own components and children (if any) following the sampling routine stated as above. 

% \todo{add an algorithm or an example? }

% How we design the sampling probability and how we sample operators \& operants from the possibility space. 

\subsubsection{Space evaluation} 

\begin{table*}[t]
    \centering
    \caption{\footnotesize Selected matrices calculation process. For some notations used, $F$ is the flow matrix. $P$ is the original coordinate matrix before rigid motion transformation. $N$ is the normal matrix.  $\overline{M}$ is matrix after centralizing $M$. ``Decompose Res.'' means that the expected vector is one of the SVD decomposed right singular vectors (always the one of the most smallest singular value). 
    % column vector of the SVD decomposed right singular matrix 
    } 

    \begin{tabular}{@{\;}c@{\;}|c|c|c@{\;}}
    \midrule
        \hline
        \specialrule{0em}{1pt}{0pt} 
        Feature & Calculation process & Input matrices & Appendix \\ 
        \cline{1-4} 
        \specialrule{0em}{1pt}{0pt}
      
        Rotation matrix $R$ & \makecell[c]{ $\text{orth}(\text{sum}(\text{cartesian}(P + F, P)))$ } & $P, F$ & /

        \\ \cline{1-4} 
        \specialrule{0em}{1pt}{0pt}
        
        Cone apex $\vec{c}$ & $\text{sum}(\text{cartesian}(N^{+T}, \text{rowsum}(N\cdot P)))$ 
        % $\vec{c} = \min_{\vec{c}} \Vert N\vec{c} - \text{rowsum}(NP)\Vert_2$  
        & $N, P$ & /
        % \footnote{$N$ is the normal matrix, $P$ is the coordinate matrix.}  
        \\ \cline{1-4} 
        \specialrule{0em}{1pt}{0pt}
        
        Cone/Cylinder axis $\vec{a}$ & $\text{svd}(\overline{N})$ & $N$ & Decompose Res.
        % \footnote{$\bar{N}$ is the normal matrix after centralizing $N$.}   
        \\ \cline{1-4} 
        \specialrule{0em}{1pt}{0pt}
        
        Sphere center $\vec{c}$ & $\text{sum}(\text{cartesian}((-2\overline{P})^{+T}, \text{rowsum}(P^2)))$ 
        % $\vec{c} = \min_{\vec{c}} \Vert -2\bar{P}\vec{c} - \bar{\text{rowsum}(P^2)} \Vert_2$ 
        & $P$ & /   \\ \cline{1-4} 
        \specialrule{0em}{1pt}{0pt}
        
        Sphere radius $r$ & $r = \text{sqrt}(\text{mean}(\text{P} - \vec{c})^2)$ & $P, \vec{c}$ & /   \\ \cline{1-4} 
        \specialrule{0em}{1pt}{0pt}
        
        Plane normal $\vec{n}$ & $\text{svd}(\overline{P})$ 
        % $\vec{n} = \min_{\vec{n}} \Vert \bar{P} \vec{n} \Vert_2$ 
        & $P$ & Decompose Res. \\   \cline{1-4} 
        \specialrule{0em}{1pt}{0pt}
        
        % Plane offset $d$ & $d = \text{mean}(P\vec{n})$ & $P, \vec{n}$ & / \\   \cline{1-4} 
        % \specialrule{0em}{1pt}{0pt}

    \end{tabular} 
    \label{tb_feat_calculation}
\end{table*} 

As stated above, our operation space is constructed based on simple feature set level grouping operations and point-level feature operations, which are quite simple compared with the carefully designed features specifically for a single task which are used to guide the network to learn the task properly. 

However, many of such features can be generated from such an operation space as shown in Table~\ref{tb_feat_calculation}. 


\subsection{Conditional operation sampling and space optimization}

After the operation space is constructed, we fit it to each specific part segmentation task for their own operation preference. In this process, we adopt a propose, evaluate and update process by sampling operations from the operation space, putting them under a simulated domain generalization setting to evaluate its generalization ability and then update the operation space by evaluation metric obtained in the evaluation stage. 

We then introduce such three stages in detail as follows. 

% \todo{an overview of the propose, evaluate and optimize process}

\subsubsection{Operation tree sampling}

The operation tree that generating the supervision target is sampled in a top-down manner by sampling operators for each cell and its following children cells layer-by-layer. 

To be more specific, we perform the conditional sampling process for each kinds of operation cells in the following routines: 
\begin{itemize}
    \item Mid-level operation cell: 1). Sample its unary operator $u$ from the corresponding unary operator distribution; 2). Sample its grouping operator $g$ conditioned on the sampled $u$ for the corresponding grouping operator distribution. Different uanry operators will not share their grouping operator distributions. 3). Sample which children to continue conditioned on the sampled unary operator and grouping operator combination $(u,g)$. 
    \item Leaf-level operation cell: 1). Sample its unary operator $u$ from the corresponding uanry operator distribution; 2). Sample its operant $f$ conditioned on the sampled $u$ form the operant sampling distribution specifically for $u$. 
\end{itemize}

We then give an example to illustrate the sampling process and the probability calculation. 
Suppose an operation tree is sampled as following: 
\begin{flalign*}
    \{ u_1^3, g_1^3, b_1^3, lc &: \{ u_2^1, f_2^1 \}, \\ 
    rc &: \{ u_3^2, g_3^2, b_3^2, lc : \{ u_4^1, f_4^1 \},
    rc : \{ u_5^1, f_5^1 \} \}\},
\end{flalign*}
where the subscription indicates the cell number, while the superscription denotes the cell level (level $1$ for leaf cells); $rc$ ($lc$) denotes the right (left) child.
The probability density value is the calculated as: 
\begin{align}
    g = g(c_1^3)g(c_2^2 | c_1^3)g(c_3^2 | c_1^3)g(c_4^1 | c_3^2, c_1^3)g(c_5^1 | c_3^2, c_1^3),
\end{align}
where 
\begin{align}
    p(c_1^3) &= p(u_1^3)p(g_1^3 | u_1^3)p(b_1^3 | g_1^3, u_1^3) \\ 
    p(c_2^2 | c_1^3) &= p(u_2^1 | c_1^3)p(f_2^1 | u_2^1, c_1^3) \\ 
    p(c_3^2 | c_1^3) &= p(u_3^2 | c_1^3)p(g_3^2 | u_3^2, c_1^3)p(b_3^2 | g_3^2, u_3^2, c_1^3) \\ 
    p(c_4^1 | c_3^2, c_1^3) &= p(u_4^1 | c_3^2, c_1^3)p(f_4^1 | u_4^1, c_3^2, c_1^3) \\ 
    p(c_5^1 | c_3^2, c_1^3) &= p(u_5^1 | c_3^2, c_1^3)p(f_5^1 | c_3^2, c_1^3).
\end{align}
Each probability distribution is a multinomial distribution in our implementation. 

% \todo{add an example and PDF}

% After the supervision target generation tree is constructed, we sample supervision targets from it in a top-down manner, where the operators sampled in shallower level nodes will determine on which node in the next level should the sampling process continue. 

% Specifically, suppose the sampled operator sequence is \{$\mathcal{S}_1, \mathcal{S}_{2l}, \mathcal{S}_{2r}, \mathcal{S}_{3l}, \mathcal{S}_{3r}$\}, where $\mathcal{S}_{i(l/r)}$ denotes the operator set sampled in the (left/right) i-th level node. 
% The probability density value of such result is as follows:

% \begin{align}
%     &g(\mathcal{S}_1, \mathcal{S}_{2l}, \mathcal{S}_{2r}, \mathcal{S}_{3}) \\ &= g(\mathcal{S}_1)g(\mathcal{S}_{2l} | \mathcal{S}_1)g(\mathcal{S}_{2r} | \mathcal{S}_1)g(\mathcal{S}_{3l} | \mathcal{S}_1, \mathcal{S}_{2l}) g(\mathcal{S}_{3r} | \mathcal{S}_1, \mathcal{S}_{2r}). 
% \end{align}

\subsubsection{Supervision target evaluation} 
The supervision target sampled from the operation space is then evaluated by plugging it to the segmentation framework and optimizing the l2 loss between the sampled target and the transformed per-point intermediate representation. 
A cross-validation approach is used to estimate the generalization ability of the generated supervision target under a simulated domain generalization setting. 
After that, the average generalization gap over all splits is taken as the reward for further space optimization. 


\subsubsection{Operation space optimization}

The operation optimization process is derived from the REINFORCE~\cite{williams1992simple} algorithm. 
Given a sampled operation sequence $\mathcal{S}$ and its corresponding reward $r$, we optimize each sampling distribution involved in the sampling process of $\mathcal{S}$ by related distribution parameter $w_i^j$ via: 
\begin{align}
    w_i^{jk\prime} &= w_i^{jk} - \Delta w_i^{jk} \\ 
         &= w_i^{jk} - \alpha_i^{jk}(r - b_i^{jk})e_i^{jk} \\ 
         &= w_i^{jk} - \alpha_i^{jk}(r - b_i^{jk})\frac{\partial\ln  g}{\partial w_i^{jk}},
\end{align}
where the subscription denotes the number of cell, while the first  superscription indicates index of the cell node which the current weight belongs to, the second one is the index of the weight value in the cell node $k$. 

The value of $\frac{\partial \ln g}{\partial w_i^{jk}}$ can be simply calculated by 
\begin{align}
    \frac{\partial \ln g}{\partial w_i^{jk}} = \frac{\partial \ln g(w_i^{jk} | w_i^{j-1}...w_i^{1}, c_{i-1}, ..., c_i)}{\partial w_i^{jk}}
\end{align}
since $g$ can be decomposed into a sequence of multiplication of conditional distributions. Each conditional distribution here is a multinomial distribution as stated above, the  log-probability density of sampling a value from such distribution can be easily calculated by the class function ``log\_prob'' of the corresponding Pytorch Distribution module. 

% To optimize the supervision target generation space, or operator and operants sampling distributions, specifically, we adopt the REINFORCE~\cite{williams1992simple} algorithm by via a proposing, evaluating and updating routine. 

% In detail, we draw $k$ samples from the target generation space by sampling formulas from it in each epoch. 
% Then we adopt a $m$-fold cross-validation approach to evaluate the effectiveness of such $k$ supervision targets: 1). The train set into $m$ subsets with relatively obvious distribution gap among each other to simulate domain shift. 2). For each sampled supervision target, we evaluate its cross-domain generalization performance by training $m$ models on $m-1$ domains and evaluating on the left-out domain. 3). We take the average evaluation metric gap between the left-out validation domain and the training domains over such $m$ evaluation process as the reward value, which is then used to update the supervision target generation space. 

% As for the detailed distribution optimization strategy, we sample 
% The optimization strategy is derived from the REINFORCE algorithm, where each parameter $w_{i}$ that counts in the sampling process is updated by minusing its corresponding $\Delta w_{i} = \alpha_{i}(r - b_{i})e_i$, where $e_{i} = \partial \ln g / \partial w_{i}$, $g$ is the probability density function. 
% Thus, $e_{i}$ for parameter $w_{i}$ of each distribution lying in node of each level can be derived as: 

% \begin{align}
%     e_i &= \frac{\partial g}{\partial w_i} \\ 
%     &= \frac{\partial \ln( g(\text{H})g(v| \text{H})g(\text{L}|\text{H},v) )}{\partial w_i} \\
%     &= \frac{\partial \ln(g(\text{H})  + \partial \ln(g(v| \text{H})) + \partial  \ln(g(\text{L} | \text{H},v)) )} {\partial w_i} \\
%     &= \frac{\partial \ln(g(v| \text{H})}{\partial w_i},
% \end{align}

% where $g(\text{H})$ is the probability density of values sampled in upper layers, $g(\text{L} | \text{H}, v)$ is the probability density of values sampled in lower layers conditioned on the current sampled value $v$ and those sampled in upper layers $\text{H}$, which are not relevant with the sampling distribution in the current layer resulting value $v$. The conditional distribution for each sample $g(v| \text{H})$ is a multinomial distribution, in our implementation, which can be simply calculated by the class function ``log\_prob'' of the corresponding Pytorch Distribution module. 

% Propose, evaluate and update distribution
% \begin{itemize}
%     % \item Reward design ---- generalization gap and cross validation
%     \item The REINFORCE algorithm
%     \item The simple updating process is accepted by REINFORCE algorithm
% \end{itemize}


\subsection{Greedy supervision targets selection}

% After the operation space is optimized, we can get a series of distributions from the operation space, which are further used to propose multiple supervision target formula

\begin{algorithm}[H]
% \algsetup{linenosize=\tiny}
\small %\small, \footnotesize, \scriptsize, or \tiny
\caption{SortedByCrossVal. 
}
\label{algo_sorted_by_cross_val}
\footnotesize
    \begin{algorithmic}[1]
        \Require
            The model $\mathcal{M}$; Split train set $\mathcal{S}_{sp} = \{ \mathcal{S}_1, \mathcal{S}_2, ..., \mathcal{S}_k \}$; A set of intermediate supervision targets $\mathcal{T} = \{t_1, t_2, ..., t_K\}$.
            % Input graph $G(\mathcal{V}, \mathcal{E}, \mathbf{X})$; The model $\mathcal{M}$;  Masking steps $T$; The number of nodes for masking at each step $\alpha$.
            % Graph encoder $\text{GNN}(\cdot)$ and node classifier $f(\cdot)$;
        \Ensure
            % Masked node set $\mathcal{S}$; 
            Sorted intermediate supervision targets $\mathcal{T}'$.
            % Selected intermediate supervision target set $\mathcal{T}_s = \{t_{s1}, ..., t_{sk} \}, 1\le k \le 3$. 
        
        \For{$i = 1$ to $\vert\mathcal{T}\vert$}
            \State $s \leftarrow \text{Cross\_Val}(\mathcal{M}, \mathcal{T}_1[i], \mathcal{S}_{sp})$
            \State $\mathcal{T}_1[i] \leftarrow (\mathcal{T}_1[i], s)$
        \EndFor
        
        \State $\mathcal{T}' \leftarrow \text{sorted}(\mathcal{T})$
        \Return $\mathcal{T}'$
       
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
% \algsetup{linenosize=\tiny}
\small %\small, \footnotesize, \scriptsize, or \tiny
\caption{Greedy Supervision Selection. 
}
\label{algo_greedy_sel}
\footnotesize
    \begin{algorithmic}[1]
        \Require
            The model $\mathcal{M}$; Split train set $\mathcal{S}_{sp} = \{ \mathcal{S}_1, \mathcal{S}_2, ..., \mathcal{S}_k \}$; A set of sampled intermediate supervision targets $\mathcal{T} = \{t_1, t_2, ..., t_K\}$.
            % Input graph $G(\mathcal{V}, \mathcal{E}, \mathbf{X})$; The model $\mathcal{M}$;  Masking steps $T$; The number of nodes for masking at each step $\alpha$.
            % Graph encoder $\text{GNN}(\cdot)$ and node classifier $f(\cdot)$;
        \Ensure
            % Masked node set $\mathcal{S}$; 
            Selected intermediate supervision target set $\mathcal{T}_s = \{t_{s1}, ..., t_{sk} \}, 1\le k \le 3$. 
        
        \State $\mathcal{T}_1 \leftarrow \mathcal{T} $
        \State $\mathcal{T}_1 \leftarrow \text{SortedByCrossVal}(\mathcal{M}, \mathcal{T}_1, \mathcal{S}_{sp})$
        % \For{$i = 1$ to $\vert\mathcal{T}_1\vert$}
        %     \State $s \leftarrow \text{Cross\_Val}(\mathcal{M}, \mathcal{T}_1[i], \mathcal{S}_{sp})$
        %     \State $\mathcal{T}_1[i] \leftarrow (\mathcal{T}_1[i], s)$
        % \EndFor
        % \State $\mathcal{T}_1 \leftarrow \text{sorted}(\mathcal{T}_1)$
        \State $\mathcal{T}_2 \leftarrow \mathcal{T}_1[1: 2] \times \mathcal{T}_1[1: \vert \mathcal{T}_1 \vert / 2]$
        \State $\mathcal{T}_2 \leftarrow \text{SortedByCrossVal}(\mathcal{M}, \mathcal{T}_2, \mathcal{S}_{sp})$
        \State $\mathcal{T}_3 \leftarrow \mathcal{T}_2[1: 3] \times \mathcal{T}_1[1: \vert \mathcal{T}_1\vert / 3]$
        \State $\mathcal{T}_3 \leftarrow \text{SortedByCrossVal}(\mathcal{M}, \mathcal{T}_3, \mathcal{S}_{sp})$
        \State $\mathcal{T}_s \leftarrow \text{sorted}(\{\mathcal{T}_1[1], \mathcal{T}_2[1], \mathcal{T}_3[1] \})[1]$ \\ 
        \Return $\mathcal{T}_s$
       
    \end{algorithmic}
\end{algorithm}

Based on the operation space optimized in the training stage, we adopt a beam search like strategy to select which target combination to use in the further evaluation stage. 
Simply speaking, we select the combination containing at most three supervision targets by estimate their generalization ability under a cross validation setting simulated by cross validating the split training domains. 
To be more specific, this process is performed in the following steps: 
\begin{itemize}
    \item Cross-validate the performance of a single supervision target and rank them to get an ordered set $\mathcal{S}_1$ according to their performance; 
    \item Pick first two formula from $\mathcal{S}_1$ and combine them with the Top-$\vert \mathcal{S}_1 \vert / 2$ formula to get $\vert \mathcal{S}_1 \vert - 1$ combinations, each element in which is combined of two supervision target formula. Then such $\vert \mathcal{S}_1 \vert - 1$ combinations are cross-validated and then further ranked according to their estimated generalization ability. Such an ordered set is denoted as $\mathcal{S}_2$. 
    \item Pick first three formula combinations from the ordered set $\mathcal{S}_2$ and combine them with the first $\vert \mathcal{S}_1 \vert / 3$ targets from $\mathcal{S}_1$ to get roughly $\vert \mathcal{S} \vert$ combinations, each element in which is combined of three supervision target formula. Then such combinations are further ranked based on their estimated generalization ability. Denote the ordered set as $\mathcal{S}_3$. 
    \item The supervision target combination from the union set $\mathcal{S} = \mathcal{S}_1 \cup \mathcal{S}_2 \cup \mathcal{S}_3$ that achieves the best cross-validation result is used in the following evaluation process for the final result. 
\end{itemize}

The selection process is also summarized in Algorithm~\ref{algo_greedy_sel}.

% Select which combination to use from the distribution updated in the optimization process
% \begin{itemize}
%     \item Greedy beam search
% \end{itemize}



==> articles/old/related_old.tex <==
% !TEX root = ../main.tex

\section{Related Work}
% Our work addresses the generalization problem of deep learning models on 3D part segmentation tasks by automatically searching intermediate supervisions, which is related to previous domain generalization strategies, 3D part segmentation task-specific approaches, and metric learning methods.

\subsection{Domain Generalization}
Most deep learning algorithms rely on the assumption that the source and target data are independent and identically distributed (i.i.d.). However, in practical applications, it is more common when the target data comes from a distribution different from that of the source data, which is addressed as the out-of-distribution (OOD) scenarios. Among the extensive efforts devoted to improving OOD generalization performance of deep learning models, domain generalization (DG) methods learn a model with data from multiple source domains such that the model can generalize well to an unseen domain. In recent years, DG has been attracting increasing attentions from researchers and various methods have been proposed to tackle this issue. Previous works on DG can be classified into mainly four categories according to the strategies they employ: 1) learning domain invariant features from multiple source domains, which includes domain alignment methods that aim to minimize the difference between source domains\cite{pmlr-v28-muandet13,li2018domain,li2018deep}, meta-learning methods that expose model to domain shift during training \cite{li2018learning,li2019episodic}, and other model-agnostic strategies\cite{Mansilla_2021_ICCV}, 2) data augmentation algorithms to simulate domain shift \cite{zhou2021domain}, 3) ensemble learning technique that trains domain-specific models and uses their ensemble for inference\cite{xu2014exploiting,zhou2021domain}, 4) automated machine learning (AutoML) techniques that aim to automatically search for data augmentation\cite{cubuk2019autoaugment,li2020dada} or neural architecture\cite{bai2021ood,pmlr-v70-cortes17a} which can achieve optimal generalization performance. In this work, we are interested in automatically searching for intermediate supervision to extract domain invariant features.
%\eric{Talk about the role of AutoML in DG (search data augmentation, search architecture, etc.).}

\subsection{3D Part Segmentation}
We demonstrate the effectiveness of \gps on three 3D part segmentation tasks, namely motion segmentation, primitive fitting and instance segmentation, and thus we first give a brief overview on previous approaches employed for these tasks.

\subsubsection{Motion Segmentation}
% part-mobility parsing is important; segment parts by their mobility is important?
In the motion segmentation task, articulated input objects are parsed into rigidly moving parts. 
Interpreting 3D objects by their moving parts is crucial basic task of many vision, robotic and HOI (Human-Object Interaction) tasks such as object functionality understanding.
A number of previous works have devoted into solving such a problem based on traditional technologies such as traditional clustering~\cite{tzionas2016reconstructing,yuan2016space} as well as neural networks thanks to the quick development of deep learning in 3D vision community~\cite{yi2018deep,hu2017learning}. 


\subsubsection{Primitive Fitting}
Primitive fitting addresses the task of clustering input points and fitting them with geometric primitives. Standard solutions for primitive fitting tasks include RANSAC\cite{schnabel2007efficient} and region growing\cite{marshall2001robust}. As deep learning techniques have been applied widely in recent years, supervised\cite{li2019supervised,Yan_2021_ICCV,huang2021primitivenet} and unsupervised\cite{tulsiani2017learning,fang2018planar} learning-based primitive fitting algorithms have been proposed.\cite{li2019supervised} proposes an end-to-end neural network that takes point clouds as input and predicts a varying number of primitives. \cite{Yan_2021_ICCV} further uses hybrid feature representations to separate points of different primitives. However, to extract accurate features from point clouds and achieve high primitive fitting performance, previous task-specific methods employ sophisticated framework and delicately designed supervisions. On the contrary, \gps uses simple backbone and automatically searches for features to learn, while achieving competitive generalization result.

\subsubsection{Instance Segmentation}
Instance segmentation is a fundamental task in many vision systems. 
Traditional strategies proposed to solve this problem always tend to heuristically design geometric criterion for segmenting shapes, including K-means~\cite{shlafman2002metamorphosis}, graph cuts~\cite{golovinskiy2008randomized}, spectral clustering~\cite{liu2004segmentation}, to name a few. 
Such strategies always work on 3D meshes, with relatively rich point-level information such as per-point normal as well as point-point connectivity information. 
With the development of deep learning techniques, a wide range of learning based strategies have been proposed for part segmentation~\cite{qi2017pointnet,yi2019gspn}.
Learning based strategies, although could always get state-of-the-art performance on shapes from seen categories, are hard to take category variant information to do solve the problem, indicating their hard to parse shapes from a unseen category, as observed in~\cite{luo2020learning}. 
In this work, we also adopt the zero-shot instance segmentation setting. 
We would demonstrate that, using simple learning based frameworks designed for 3D point cloud equipped with intermediate supervisions searched for this task by the proposed \gps, we are able to get comparable performance to the previous literature. 


\subsection{Auxiliary Supervision}
% \eric{Talk about common regularizations (e.g. weight decay), multi-task learning, label encoding and compare ours with these.}
Adding auxiliary supervisions is a common strategies adopted by previous works which can help improve the performance of the network, better regularize the network's learning process, etc. 
Among them, weight decay is a widely used strategy to improve the generalization ability of neural networks~\cite{krogh1992simple,loshchilov2017decoupled}; multi-task learning (MTL) trains a network to solve multiple tasks by sharing parameters between different tasks, where the performance and the generalization ability of interested branches could benefit from other branches~\cite{crawshaw2020multi,zhang2017survey,he2017mask,ren2015faster}; Deeply Supervise~\cite{lee2015deeply} and Inception~\cite{szegedy2015going} explores how to add auxiliary supervisions on hidden layers which can help improve the quality of learned low-level features~\cite{zhao2017pyramid,zhang2018exfuse}; LabelEnc~\cite{hao2020labelenc} proposes a new label encoding function to map ground-truth labels to the latent embedding space to add auxiliary supervisions for the model's learning process. 

In this work, we also lay great importance on the role of intermediate supervisions in the segmentation networks' learning process. 
We propose to select what intermediate supervisions to add for a better generalizable network by finding suitable features to predict automatically. 
Such intermediate supervisions can be viewed a regularization method to help the network learn more domain invariant features. 
Similar with~\cite{hao2020labelenc}, ground-truth labels are also considered in the intermediate supervision targets generation process. 
